Attentional Heterogeneous Graph Neural Network: Application to Program Reidentification

Program or process is an integral part of almost every IT/OT system. Can we trust the identity/ID (e.g., executable name) of the program? To avoid detection, malware may disguise itself using the ID of a legitimate program, and a system tool (e.g., PowerShell) used by the attackers may have the fake ID of another common software, which is less sensitive. However, existing intrusion detection techniques often overlook this critical program reidentification problem (i.e., checking the program's identity). In this paper, we propose an attentional heterogeneous graph neural network model (DeepHGNN) to verify the program's identity based on its system behaviors. The key idea is to leverage the representation learning of the heterogeneous program behavior graph to guide the reidentification process. We formulate the program reidentification as a graph classification problem and develop an effective attentional heterogeneous graph embedding algorithm to solve it. Extensive experiments --- using real-world enterprise monitoring data and real attacks --- demonstrate the effectiveness of DeepHGNN across multiple popular metrics and the robustness to the normal dynamic changes like program version upgrades.

==> bk/01-intro.tex <==
\section{Introduction}
% With computers and networked systems playing indispensable roles in almost every aspect of modern society such as industry, government, and economy, cyber security undoubtedly bears the utmost importance in preserving right social orders. 

% Security problem background.
% (1)Security fact.
% (2)Introduce traditional malicious program analysis 
% (3)Introduce the most common studied problem: malware detection, which is a binary classification problem.

% Introduce our newly formulated problem--program re-id.
% (1) drawback of malware detection: (a) too less malware sample (b) highly rely on the sandbox and takes long time anlysis (c) can not deal with unknown program (d) not robust to version upgrade
% (2) the reason to formulate the new problem
% (3) introduce the new problem and proposed approach
% (program plays the key role and it is the only system entity which can embedded hacker's malicious logic. Thus to detect the hacker's malicious behavior, we need to identify malicious program.
% Similar to person Re-ID problem, each program also has its own ID (normally its exename). It is necessary to check whether its ID matches its normal behavior or not to verify that it is really the one that it claimed itself to be. If it doesn't match, it is much more likely to have some problem. We should perform further analysis and matched with the database.)

% Introduce the application
% (1) Disguised program detection
% (2) Malicious program detection
% (3) Program update robustness


Modern enterprises often rely on \acf{ids}, either misuse-based or anomaly detection based, to protect their IT and OT systems. However, existing \ac{ids} techniques overlook one critical problem, which is the \problem: given a program, with a claimed ID (such as executable name), running in the system, can we confirm the program's identity and guarantee that this program is not a disguised malicious program, or a hijacked program with different behaviors, by comparing it to the normal program with the same ID? To make the attack processes stealthy and avoid detection, adversaries often falsify the IDs of the tools they have used to bypass the \ac{ids}. For example, %a malware can disguise itself as a legitimate program
a malware may have the ID of a benign software~\cite{liu2018towards} and a system tool (\textit{e.g.}, PowerShell) used by the adversaries may have the ID of another software which is less sensitive~\cite{powershellinject}. In fact, running programs with fake IDs is a strong signal of the system being compromised~\cite{gao2018saql}. Capturing the programs with fake IDs can help identifying very stealthy attacks and reduce the security risks in enterprise networks. 



\nop{In order to avoid detection, malware can disguise
itself as a legitimate program or hijack system processes to reach
its goals. Commonly used signature-based Intrusion Detection
Systems (IDS) struggle to distinguish between these processes
and are thus only of limited use to detect such attacks. They also
have the shortcoming that they need to be updated frequently to
possess the latest malware definitions. This makes them inherently
prone to missing novel attack techniques. Misuse detection IDSs
however overcome this problem by maintaining a ground truth
of normal application behavior while reporting deviations as
anomalies.

There are many ways malware can avoid detection. One
such way is to disguise itself as a legitimate program or to
hijack system processes to reach its goals. This can start with
the visit of an infected website that exploits a vulnerability
in a browser plug-in [1], [2] and ranges over legitimate
downloads infected via a man-in-the-middle attack [3]. A
common technique to prevent plug-in based intrusion is sandboxing
of browser tabs [4]. Anti-virus software widely uses
signature based detection [5] to recognize infected executables
among incoming files. And several approaches to profile user
activities and detect deviation from normal behavior have been
established under the topic of continuous authentication [6],
[7], [8] as well as insider threat detection [9], [10].
A common detection evasion technique for malware is to
disguise itself as another process, either by hiding inside the
application’s binary or through direct impersonation
}


Existing techniques cannot be directly applied to address the problem of \problem. Digital code signing techniques, such as Public Key Infrastructure (PKI)~\cite{pki}, may help identify the certified authors of programs. However, many open-source programs that are widely used in enterprises may not contain valid signatures. Further, modern programs are evolving at a fast pace. Each version of the program has a unique signature. Handling the fast inflating set of signatures for programs is practically difficult. Malware detection or Anti-Virus~\cite{Zhang:2014:SAM:2660267.2660359,yuan2014droid,nissim2014novel} may detect malware. Yet, adversaries may also use common system tools to finish their attacks, such as malware free attacks~\cite{zimba2017malware}. Besides, a sophisticated malware can also bypass the anti-virus by hiding its malicious features and an adversary can also hijack the memory of a benign program to perform malicious actions~\cite{arefi2018faros}. There are more sophisticated program watermarking techniques to identify a program~\cite{ren2014droidmarking,ma2015software,venkatesan2001graph}, but their computational costs are prohibitively high so that they cannot be widely applied to modern enterprise environments, which contain millions of programs.


% Public Key Infrastructure (PKI)~\cite{pki} which  




% or host intrusion detection~\cite{} techniques

% With IT and OT systems playing indispensable roles in almost every aspect of modern society, such as industry, government, and economy, everything runs on program/process, including many critical missions. Can we trust these programs, executed, either deliberately or in the background, not to perform unwanted or harmful actions? %However, programs that appear to come from reputable publishers, often breach our trust by performing some unwanted or harmful actions. 
%  %\myred{Google and add some examples} 
% %For example, some programs are embedded with adware, which is designed to inset advertisements onto software packages in order to drive revenue through page view. In worst case, it hides the destructive malware. 
% %With IT and OT systems widely deployed to manage the business in industry, government, and economy, cyber-security undoubtedly bears the utmost importance in preserving right social orders. However,nowadays, serious cyber-attacks keep happening, which causes significant financial loss and public tensions.

% To establish trust in third-party programs, an intrusion detection system, either misuse-based or anomaly-based, is often applied to keep track of the running status of the entire network and identify programs that are associated with potential attacks or malicious  behaviours. Misuse detection~\cite{jones2000computer} requires the system to be aware of malicious behavior patterns prior to the actual attack. While anomaly detection techniques~\cite{mutz2006anomalous,hofmeyr1998intrusion} can be more effective and allow for detecting novel attacks, unfortunately, these approaches are prone to generate high rates of false alarms~\cite{spathoulas2009usin,airrtea}. According to a recent study conducted by FireEye, most organizations receive $17,000$ alerts per week with more than 51\% of them are false positives~\cite{hmaitmth}. \dingli{ intrusion detection is a broader concept than malware detection. I feel we should not put them together. Malware detection roughly equals to anti-virus, it mainly uses program executable examination or process memory monitoring. Intrusion detection is more general, it evolves log analysis and network packets analysis. We can say malware detection is one type of IDS.}


% While the intrusion detection approaches still deserve their own merits, in this paper, we draw readers' attention to a slightly different, yet complementary, \textit{program identity verification} problem. Namely, given a program, with a claimed ID (such as executable name), running in the system, can we design an algorithm to confirm the program's identity and guarantee that this program is not a disguised malicious program, or an altered program with different behaviors, by comparing to the normal program with the same ID?  %In IT/OT systems, everything runs on program/process, including many critical missions. Can we trust these programs, executed, either deliberately or in the background, not to perform unwanted or harmful actions?
% \dingli{I feel one thing we are missing is why this is an important problem (as important as IDS)? Why solving this problem could help improve the security of the system? }

% \dingli{To sum it up, I feel we should still put our approach as a new IDS approach, which is complimentary to existing techniques. A program with fake identification is a signal of intrusion. However, current IDS techniques overlook such a signal. We make the first effort to capture this signal. In this case, the program identification program is important because it captures more 
% }
% To address this problem, most, if not all, of the traditional program identity verification methods rely on the code-signing Public Key Infrastructure (PKI)~\cite{pki}.



% %CARaddresses the aforementioned challenges inthree steps. To model the temporal dependencies between alerts,we design a prefix tree-based model that compactly represents alertsequences as well as preserves long-term temporal dependencies.A set of hierarchical Pitman-Yor priors are used to model the de-pendencies in a probabilistic way. We further discover a set of alertpatterns that correlate individual alerts with higher-level abnormalbehaviors. To model the content correlations between alerts, wepropose an entity embedding-based model to learn the latent vec-tor of each entity. Based on the latent representation, a proximitymeasurement is adopted to quantify the similarity between alerts.Finally, in order to simultaneously consider the temporal and con-text correlations, we propose the collaborative alert ranking viaa unified optimization framework, such that low-level alerts andhigh-level alert patterns that truly relate to abnormal behaviorscan be uncovered. Empirical studies on both synthetic and realenterprise alert data demonstrate the effectiveness of our proposedmodel
% %\myred{Add what is PKI, related work and its advantages}
% PKI is a system for the creation, storage, and distribution of digital certificates which are used to verify that a particular public key belongs to a certain process entity.  It creates digital certificates which map public keys to entities, securely stores these certificates in a central repository and revokes them if needed. With the help of PKI, the security of the key and assurance of public keys are satisfied. It provides trusted identification of third-party programs and their distributions.

% Although the traditional code signing provides some valuable ways to make the operating systems more secure, signed malware or advanced threats can still evade system protection mechanisms or anti-virus programs, which often neglect to scan the programs with signed signatures. %\myred{Add an example}
% Malware authors usually steal and sign their program with digital certificated. For example, the Stuxnet worm use device drivers that were digitally signed with keys stolen from two Taiwanese semiconductor companies to bypass the anti-virus detectors \cite{falliere2011w32}.
% \nop{In the past, compromised code-signing certificates have been associated with advanced threats, likely developed by nation-state adversaries. For example, the Stuxnet worm included device drivers that were digitally signed with keys stolen from two Taiwanese semiconductor companies, located in close proximity [10]. The
% Flame malware masqueraded as a file from Windows Update by
% conducting a previously unknown chosen-prefix collision attack
% against the MD5 cryptographic hash [33]. In both cases, the valid
% digital signatures allowed the malware to evade detection and to
% bypass anti-virus and Windows protections. TODO: Programs without signed signatures does not mean they are not secure}
% What is worse, these signed malwares often have a normal executable name to hide their real malicious intention. 
% %\myred{Add an example}  
%  \nop{When a user visits http://woofles.github.io/placeholder/infector/ to play a seemingly harmless game, they are informed their Java version is out of date and prompted to download and install a Java update. When the user opens the fake Java update file it will be prompted by User Account Control to allow the program to run. Since the installer was written in Java, the UAC popup will tell the user the file is signed by Oracle Corporation, so it will have a valid digital signature.}
% On Windows machines, malware authors usually use ssvchost.exe as  a  facade to attach malicious code or to name processes identically in order to avoid detection. Therefore, there exists a vital need for the methods that can verify the programs with signed signatures and disguised executable names in an effective and efficient way. 


% Fortunately, modern world has witnessed a dramatic increase in our ability to collect, transmit and distribute real-time monitoring and surveillance data from large-scale IT and OT systems, many real information networks like the enterprise networks often generate a large volume of system operational data with rich information on program/process level events. 
% The process-level events reflects the interactions between a process and another system entity (\textit{e.g.}, a process opens a file or forks another process). These low-level process events provide an opportunity for checking the process identity, in the context of process behaviors. A key question is how to exploit the massive process-level events for program identity verification. 
We observe that the system behaviors, such as file accessing, inter process communications, and network communications, of a program have distinguishable patterns~\cite{tang2018node}. Such patterns are stable during the evolution of the program and the system behavioral events can be efficiently collected by system monitoring techniques~\cite{kernelaudit,etw}. For example, every instance of excel.exe loads a fixed set of .DLL files while opening a spreadsheet file. If an excel.exe instance performs a rare operation, such as loading a unseen .DLL file or initiating another process, this excel.exe instance is very likely to be hijacked or even a malware with the ID of excel.exe.
Based on this observation, 
in this paper, we propose \ourss, a attentional multi-channel graph neural network based approach for \underline{deep} program \underline{reid}entificaion based on the system behaviors of the program. 
% system monitoring and surveillance data. 
%Specifically, to perform program identity verification efficiently and effectively, we propose a deep program identity verification approach via attentional multi-channel contextual graph encoder to generate the graph embedding of the program behavior graph. 

In particular, we design a compact graph modeling, the behavior graph, to capture the interactions between different system entities. %, and construct a Heterogeneous Information Network (HIN). 
This graph modeling effectively addresses three challenges (\textit{i.e.}, high volume, high dimension, and categorical) of the system event data and provides the foundation for further graph based program behavior analysis. %Then, we develop a machine learning model to automatically learn the patterns of system behaviors of a program from the behavior graph. To the best of our knowledge, \ourss~is the very first approach that tries to address the \problem\ in an efficient and effective manner. 
%Learning the patterns from the behavior graphs, which is an HIN, is challenging. 
The constructed behavior graph is a heterogeneous graph~\cite{shi2017survey}, which involves a hierarchy of different dependencies from simple to complex. %The behavior graph involves a hierarchy of different dependencies from simple to complex. 
Among all the dependencies, the complex ones are not exposed directly by the edges in the graph, but can be inferred by a hierarchy of deep representation. %For example, a process accessing a file (P $\rightarrow$ F) is a simple dependency, two processes  accessing the same file (P $\rightarrow$ F $\leftarrow$ P) is a complex dependency. The complex dependency can not be modeled directly with shallow representation such as simple dependency, but a hierarchy of deep representation, from simple dependency (P $\rightarrow$ F) to (P $\rightarrow$ F $\leftarrow$ P). 
\nop{To handle the complex and obscure dependencies, we need a deep graph structure learning model to capture the hierarchical dependency. However, recent deep graph structure learning methods~\cite{kipf2016semi,defferrard2016convolutional,bruna2013spectral,hamilton2017inductive,velickovic2017graph} only works for homogeneous undirected graph and can not capture the heterogeneity of \textbf{HIN}.} 
%To address this challenge, an attentional multi-channel contextual graph encoder is proposed to generate the graph embedding of the program behavior graph. 
To make the heterogeneous graph learnable via a deep representation learning, we propose a multi-channel transformation module to transform the heterogeneous graph to multiple channels of homogeneous graphs guided by the meta-paths. 
%To leverage the information of each entity, we extract the knowledge-free graph features. 
After the multi-channel transformation, we feed the multi-channel homogeneous graphs and their corresponding entity features into a graph neural network for graph embedding. 
%However, each homogeneous graph is directed, adapting existing graph neural networks directly fails to capture the directed dependency. To address this challenge, 
We propose a contextual graph encoder and stack it layer by layer to learn the hierarchical graph embedding via propagating the contextual information. Noticing the different importance of the different channels, channel-aware attention is further developed to joint the multi-channel graph embeddings.   
We conduct an extensive set of experiments on real-world enterprise monitoring data to evaluate the performance of our approach. The results demonstrate the effectiveness and efficiency of our proposed algorithm. We also apply \ourss\ to real enterprise security systems. The results show our method is effective in identifying the disguised signed programs and robust to the normal dynamic changes like program version upgrade.

%To this end, we formulate the program identity verification as a program binary classification problem: given a program with corresponding behavior data and claimed name, we verify whether it belongs to the claimed program. Specifically, to perform program identity verification efficiently and effectively, we propose a deep program identity verification approach via attentional multi-channel contextual neural encoder to generate the embedding of the program behavior graph.
%CAR addresses the aforementioned challenges inthree steps. To model the temporal dependencies between alerts,we design a prefix tree-based model that compactly represents alertsequences as well as preserves long-term temporal dependencies.A set of hierarchical Pitman-Yor priors are used to model the de-pendencies in a probabilistic way. We further discover a set of alertpatterns that correlate individual alerts with higher-level abnormalbehaviors. To model the content correlations between alerts, wepropose an entity embedding-based model to learn the latent vec-tor of each entity. Based on the latent representation, a proximitymeasurement is adopted to quantify the similarity between alerts.Finally, in order to simultaneously consider the temporal and con-text correlations, we propose the collaborative alert ranking viaa unified optimization framework, such that low-level alerts andhigh-level alert patterns that truly relate to abnormal behaviorscan be uncovered. Empirical studies on both synthetic and realenterprise alert data demonstrate the effectiveness of our proposedmodel


%\myred{Add description, novelties, and contributions of our method: how do we convert the program identity verification to a graph classification problem; how do we exploit the low-level process events}
%The primary element of program's surveillance data is the low-level system event. It consists of a program process, a destination system entity, their causal dependency and corresponding attributes. These data 
%The system surveillance data is usually high volume, high dimension and categorical, %which is difficult to use directly without any domain knowledge.
%Fortunately, it is nature to construct a behavior graph from low-level system event within a time windows. It motivates us to formulate program behavior analysis as a graph mining problem. Given a program with corresponding surveillance behavior data and claimed name, we verify whether it belongs to the claimed program or not. Specifically, we formulate it as a graph classification problem.

%Due to the unique characteristic of surveillance data, the constructed graph has two special proprieties: heterogeneous and directed.  There exists a variety type of events with variety type of destination system entities, which means the constructed graph is a heterogeneous information network (HIN). Since each event is on-way causality, the link of the graph is directed. To capture the heterogeneous and directed graph structure, we develop an novel multi-channl attentional graph embedding algorithm.  Specifically, we propose a multi-channel transformation module to transform the constructed HIN to multi-channel graph with each channel of graph being homogeneous with the guide of meta-path. It transforms the HIN mining problem to multi-view homogeneous graph mining. Though each channel of graph is homogeneous, there still exits the directed link. To learn good representation from these directed graphs, we proposed contextual neural encoder, a graph neural network, to extract the low dimensional representations by modeling the inbound and outbound connection separately. Furthermore, noticing the different importance of different channels, channel-aware attention, an  attention  mechanisms  is  proposed  to  align  the learned graph embeddings from different channels and generate the attentional joint embedding.

\nop{IT/IoT systems are widely deployed to manage the business in industry and government. Ensuring the proper functioning of these systems is critical to the execution of the business. For example, if a system is compromised, the security of the customer data cannot be guaranteed; if certain components of a system have failures, the services hosted in the system may be interrupted. 

\nop{Maintaining the proper functioning of computer systems is a challenging task. System experts have limited visibility into systems and usually give a partial view of the complex systems. This motivates the recent trend of leveraging system monitoring logs to offer intelligence in system management.} 

There are multiple type of entities in the the computer system, such as program/process, file, internet socket and so on. Among all of these entities, the program/process play a key role. It is the subject of most system event and is the only entity can embedded abnormal logic. Therefore, it required to track the behavior of the program/process to keep the safety and stability of the computer system. In computer vision, there is a task called face verification. Given a face image, it searches in a gallery for images that belongs to the same person. Motivates by face verification, we formulate the problem of the program identity verification to verify the program via its behavior. To verify a program, a naive approach is to use its binary signature. A Unique signature is generated for each known type of program, unknown program is verified by matching the its signature with existing signatures in the maintained database. However, using signature to verify the program is easily evaded by encryption, obfuscation and polymorphism. Therefore we verify the program by monitoring its behavior from its low-level system events. 

\nop{program identity verification is related to malicious program detection but benefit from more advantages. Recent years, a number of works are proposed to perform malicious program detection based on the the machine learning and data mining \cite{arp2014drebin,dimjavsevic2016evaluation,wu2014droiddolphin,saleh2017multi,hou2017hindroid}. They consider malicious program detection as a binary classification based on the program label (either malicious or benign) and the content-based feature extracted from program, such as Windows Application Programming Interfaces(APIs), system-call, n-gram binary in a statistically or dynamically way. 
program identity verification is different from malicious program detection in six folds:
%drawback of malware detection: (a) too less malware sample (b) highly rely on the sandbox and takes long time anlysis (c) can not deal with unknown program (d) not robust to version upgrade
(1) Malware detection focus on the malicious program and needs large amounts of labeled malware samples to train the model, which is difficult to obtained. Different from that, program identity verification does not require lots of malware samples, it pays attentions more on the benign programs.  
(2) Malware detection highly relies on the sandbox in form of dynamic analysis and not all malicious behaviors can appear in only one execution. Different from that, program identity verification only monitor the low-level system events in a compute system other than a sandbox.    
(3) Malware detection is highly depends on the expert knowledge. Different from that, program identity verification is expert knowledge free and in a data driven way. 
(4) Malware detection is not robust to new anomaly program. Driven by the economic benefits, malicious programs are created and being disseminated at a rate of thousands per day, making it difficult for malware detection methods to be effective. Different from that, program identity verification is capable of detection unseen malicious program samples
%as well as identifying the malware families of malicious samples.
(5) Malware detection is usually not robust to the program update. Since most of malware detection are signature-based, program update results the new signature, which can not be recognized. Different from that, program identity verification is behavior based approach, which is robust to the the program update.
(6) Malware detection is usually designed for personal computer system. Different from that, program identity verification is mainly designed for enterprise computer system, which has controlled number of programs. 
The above differences motivate us to formulate the problem of program identity verification via program behavior.}}

\nop{The primary element of program behavior is the low-level system event in a system  monitoring logs.  It consists of a program process, a destination system entity, their causal dependency and corresponding attributes. However, all of attributes are large scale and categorical, which is difficult for traditional machine learning algorithm due to lack of intrinsic proximity measures. Fortunately, it is nature to construct a behavior graph from snapshot of low-level system event within a time windows. Due to the variety of the destination system entities, there are heterogeneous types of causal dependency. Therefore, we 
%In this work, we leverage the low-level system events and 
model the program behavior as a heterogeneous information network (HIN) to capture these complex causal correlations. To efficiently and effectively encode the graph structure information, we leverage network embedding techniques and proposed a novel HIN embedding model to extract the low-dimensional representations for the HIN. To verify the given program, we determine whether its behaviors graph matches the existing known program. 
Specifically, we conduct similarity analysis in low-dimensional embedding space in a verification way.

To this end, we formulate the program identity verification as a program binary classification problem: given a program with corresponding behavior data and claimed name, we verify whether it belongs to the claimed program. Specifically, to perform program identity verification efficiently and effectively, we propose a deep program identity verification approach via attentional multi-channel contextual neural encoder to generate the embedding of the program behavior graph.}

\nop{Given a snapshots $S$ of a program with claimed name, we check whether it belongs to the claimed program. If it matches the claimed the program, the predicted label should be +1, otherwise it should be -1. Specifically, we formulate it as a binary classification problem. Given a snapshots $S$ of program, a mapping function $f$ is used to map $S$ to a binary label $Y\in \{+1,-1\}$, such that $f:S\rightarrow \{+1,-1\}$. Due to the unique characteristic of the program snapshots, we propose a multi-channel deep  graph neural network to model this mapping function.}

%To this end, we formulate the program identity verification as a program binary classification problem: given a program with corresponding behavior graph, we verify whether it similar to the known program, such that behavior graph belongs to the same program should be very similar while those belongs to the different program should be very dissimilar. Specifically, to perform similarity analysis efficiently and effectively, we propose a deep program re-identification approach via attentional multi-channel contextural neural encoder to generate the embedding of the program behavior graph.
In summary, this paper makes the following contributions:
\begin{itemize}
\vspace{-8pt}
\item %\textbf{Meaningful Newly Formulated Problem Setting} 
We identify the important problem of program reidentification in intrusion detection, which is often overlooked by the existing intrusion detection systems.
\vspace{-8pt}
\item %\textbf{Novel Graph Modeling of Program Behavior}
We propose a heterogeneous graph model to capture the interactions between different system entities from large-scale system surveillance data.
\vspace{-8pt}
\item %\textbf{Novel Multi-Channel Learning Framework for HIN}
We develop a multi-channel transformation to transform the heterogeneous information network into multi-channel homogeneous graphs. 
\vspace{-8pt}
\item %\textbf{Effective and Efficient Representation Learning from Directed Graph}
We propose a graph neural network based approach to learn the graph embedding via propagating the contextual information.
\vspace{-8pt}
\item %\textbf{Effective Channel-Aware Attention Mechanism}
We propose a channel-aware attention mechanism to jointly learn the representation from different channels. 
\vspace{-8pt}
\item %\textbf{Effective Channel-Aware Attention Mechanism}
Our empirical studies on real enterprise monitoring data demonstrate the effectiveness of our method.
\end{itemize}


\nop{
\begin{itemize}
\item \textbf{Meaningful Newly Formulated Problem Setting} 
We identify the important problem of program identity verification and propose a graph neural network solution. %To the best of our knowledge, this is the first work about graph classification on heterogeneous directed graph using graph neural networks. 
\vspace{-8pt}
\item \textbf{Novel Graph Modeling of Program Behavior}
We propose to modeling the low-level program events stream as a compact HIN from large-scale system surveillance data.
\vspace{-8pt}
\item \textbf{Novel Multi-Channel Learning Framework for HIN}
We develop multi-channel transformation to transform the HIN into multi-channel homogeneous graph. 
\vspace{-8pt}
\item \textbf{Effective and Efficient Representation Learning from Directed Graph}
We design a graph neural network based graph embedding approach--Contextual Graph Encoder to learn the graph embedding from directed graph via propagating the contextual information.
\vspace{-8pt}
\item \textbf{Effective Channel-Aware Attention Mechanism}
We propose Channel-Aware Attention Mechanism to joint the representation from different channel. 
\end{itemize}
}

\nop{In summary, this paper makes the following contributions:
\begin{itemize}
\item \textbf{Meaningful Newly Formulated \ours\ Problem Setting} 
We formulate a new problem setting--program identity verification to fill the gap of program behavior analysis, which offers the intelligence in system management and has applications to computer system security. To solve the program identity verification problem, we give a deep learning solution.

\item \textbf{Novel Graph Model of Program Behavior}
We propose to modeling the low-level program events stream as a compact HIN from large-scale system surveillance data with only categorical attributes. Moreover, we extract the expert-knowledge free feature from each entity.  

\item \textbf{Novel Multi-Channel Learning Framework for HIN}
We propose multi-channel transformation to transform the HIN into multi-channel homogeneous network. The high homogeneity is encoded across different channel. It can adapted to homogeneous network embedding method.

\item \textbf{Effective and Efficient Representation Learning from Directed Graph}
We propose a deep learning based graph embedding approach--Contextual Graph Encoder to learn the embedding from directed graph via propagating the contextual information. Different from previous methods, we consider the directed link and model the inbound and outbound connection separately.

\item \textbf{Effective Channel-Aware Attention Mechanism}
We propose Channel-Aware Attention Mechanism to joint the representation from different channel. 
\end{itemize}}

% n    this    section,we    explain    our    designof   the   overall   network   architecture   to   train   ourProgram2GraphProgram Re-ID. Specifically, it consistsof  three  stages.   First  We  get  the  required  input  pro-gram  snapshots,  then  we  generate  embedding  from  itvia feature learning, finally we optimize it vBehavior of the same program could be much differ-ent in different timestamps and machine. Such variationwithin the same program could overwhelm the variationdue to program difference and make program re-id chal-lenging,  especially in  unconstrained conditions.  Thus,it is important to jointly reduce the intra-program vari-ation  and  enlarge  the  inter-program  difference.   It  isrequired that the encoded program representation pre-serve the propriety that behavior belongs to the sameprogram are close to each other while those of differentprogram should be far away.  Therefore,  we propose alearning architecture optimized under the supervision ofmultiple tasks:  identification task and verification taskto learn such representation.  Specifically, identificationtask formulate the program re-id as a multi-class classi-fication problem, which takes full advantage of the re-ID

% abels.  It directly classifies an input program behaviorinto a large number of identity classes.  In the trainingstage, given an input program behavior with identifica-tion  supervision,  the  embedding  feature  are  extractedthough feature learning stage and then mapped to oneof a large number identities.  In the testing stage,  thelearned embedding feature can be generalized to othertask and new identities unseen in the training set.  Theidentification supervision tends to pull separate the dif-ferent  behavior  apart  and  the  learned  feature  embed-ding would have rich identity-related or inter-programvariations.  However, the identification supervision hasa  relatively  weak  constrain  on  embedding  feature  ex-tracted  from  the  same  program.   Since  dissimilar  em-bedding feature could be mapped to the same identity.This could be problematic, when generalize to new taskand new identities in the testing stage.  The verification

% In computer systems, system monitoring data are represented as temporal
% graphs. For example, in cybersecurity, system call
% (syscall) logs provide a comprehensive way to capture system
% activities [12]. Unlike its alternatives (e.g., file access
% logs [1], firewall [4], and network monitoring [23]) which provide
% partial information and are application-specific, syscall
% logs cover all interactions among system entities (e.g., processes,
% files, sockets, and pipes) over time. In Figure 1(a), a
% syscall log contains a sequence of events each of which describes
% at which time what kind of interactions happened
% between which system entities.

% program plays the key role and it is the only system entity which can embedded hacker's malicious logic. Thus to detect the hacker's malicious behavior, we need to identify malicious program.
% Similar to person Re-ID problem, each program also has its own ID (normally its exename). It is necessary to check whether its ID matches its normal behavior or not to verify that it is really the one that it claimed itself to be. If it doesn't match, it is much more likely to have some problem and should be further analyzed and matched with  with the malware database.

% Temporal graphs are key data structures used to fuse information
% from heterogeneous sources [33, 36]. In computer
% systems, system monitoring data are represented as temporal
% graphs. For example, in cybersecurity, system call
% (syscall) logs provide a comprehensive way to capture system
% activities [12]. Unlike its alternatives (e.g., file access
% logs [1], firewall [4], and network monitoring [23]) which provide
% partial information and are application-specific, syscall
% logs cover all interactions among system entities (e.g., processes,
% files, sockets, and pipes) over time. In Figure 1(a), a
% syscall log contains a sequence of events each of which describes
% at which time what kind of interactions happened
% between which system entities. Note that this syscall log
% also forms an equivalent temporal graph.





% We formulate a new problem, Program Re-ID. 

% To address the above challenges, we propose 

% Given the program event stream, for each event $e$ with process $P$, if $P$ is an unseen (new) signature with existing (old) process name, check whether the process signature and name matches, the process is really it claims to be

%In summary, this paper makes the following contributions:
% \begin{itemize}
% \item We identify the emerging problem of program re-identification via its behavior;
% \item We propose to modeling the program events stream as a compact graph to preserve its behavior from large-scale system surveillance data with only categorical attributes;
% \item We develop an deep learning framework to learn to re-identify the program in a data-driven manner;
% \item We design a multi-resolution multi-view approach to capture the high dynamic and high heterogeneity of the program behavior graph;
% \item We evaluate the proposed method on the real enterprise system and show the effectiveness of our method.
% \end{itemize}
% (1) Modeling the program events as a heterogeneous graph
% (2) Performing the Multi-Channel Transformation to capture the Heterogeneous (recent solution/xiangnan's solution)
% (3) propose a contextual neural encoder for graph embedding
% (4) use multi-resolutional augmentation augment the data or capture the dynamic
% (5) (to do): add hashing function for computational and storage efficiency
% (6) (to do): use both verification and identification objective to form the multi-task learning framework

% Experiment parts
% (1) Synthetic Experiment: evaluate on selected programs and perform binary classifications
% (2) Real World Experiment--1: evaluate on selected  malicious program to perform binary classification and get probability of each classifier 
% (3) Real World Experiment--2: evaluate on the program with different signature and verify the robustness of proposed method 

\nop{The remainder of this paper is organized as follows. Section 2 introduces preliminaries and problem statement. Section 3 presents our proposed method in detail. In Section 4, based on the real-world system surveillance data, we systematically evaluate the performance of our proposed approach in comparisons with other baseline. 
%Section 5 presents the details of system development and operation. 
Section 5 discusses the related work. Finally, Section 6 concludes.}


==> bk/02-prelim.tex <==
\section{Preliminaries and Problem Statement}
\label{sec:pre}
In this section, we first present the preliminaries, then define the machine learning problem that we are concerned with \ours. %For the following sections, we assume that the operation system is Windows System, for simplicity of explanation. 
%\subsection{Notations}

\noindent{\bf{System Entity}}
%A system entity is the basic element of the every operating system. 
There are three main types of system entities in an operating system: \textit{processes}, \textit{files}, and \textit{Internet sockets} (INETSockets). Each type of entity is associated with a set of categorical attributes. In this paper, we use ``program'' and ``process'' interchangeably whenever there is no ambiguity. %For the file entity, we use its extension name as the identifier.

\noindent{\bf{System Event}}
A system event is the interaction between a pair of system entities. Formally, a system event $e=(v_s, v_d, t)$ represents a source entity $v_s$, destination entity $v_d$ and their interaction happens at time stamp $t$. There are multiple types of system events, due to the existence of different types of entities. We consider three different types of system events, including: (1) a process forking another process (P-P), (2) a process accessing a file (P-F), and (3) a process connecting to an INETSockets (P-I). %These three types of system events model the causal dependency from a process to another system entity. Each system event is also associated with a set of attributes, including the information of the involved system entities and their dependency.

\nop{
\noindent{\bf{Program Snapshot} }
A program snapshot $S = \{e_{a_1,t_1},e_{a_2,t_1},...,e_{a_l,t_1},e_{a_l,t_2},...e_{a_l,t_m}\}$ consists of system events stream across agents $A = \{a_1, a_2, ... , a_{l}\}$ within a time period $T = \{t_1, t_2, ... , t_{m}\}$. The number of agent is denoted as $l$ and the length of time window is denoted as $m$. \myred{This definition is not clear. Snapshot only contains the events related to the specific program? If not, what else?}
}

% \subsubsection{System Behavior Graph}
% A system behavior graph is constructed from a system events snapshot. Since the system snapshot

% \subsubsection{Abnormal Program Behavior}
% Most of the abnormal program such as Trojan, Ransomware and Virus behave abnormally compared with the normal program. This kind of abnormal behaviors involve a number of low-level events to embedded the hacker's malicious logic. It is typically their system event snapshot, not individual events, that are different from normal program. We define these system events snapshot that are associated with malicious logic as abnormal program behavior.

% \subsection{Problem Statement-1}

% Given the system event data of a program contains a set of System Events Snapshot $\mathcal{S} = \{S_1,S_2,...S_N\}$, we are concerned with discovering good representation $\mathcal{H}=\{h_1,h_2,...h_N\}$ for the corresponding program system event snapshot. Specifically, we are interested in learning a representation function $f: \mathcal{S} \rightarrow \mathcal{H} $, which maps each program snapshot  $S_i \in  \mathcal{S}$ into a discriminate representation $\mathbf{h}_i \in \mathcal{H}$ can be used to identify the program in various task.
%We formulate the \ours\ as a supervised machine learning problem as follows:
%\myred{TODO:}

\noindent{\bf{Problem Statement}}
%Formally, we define our problem as followed. 
%Given a number of system snapshots $S$ of a program with claimed , we check whether the process name matches the normal behavior of claimed program and suggest the top-k program.
%Given a system snapshots $S$ of a program, we check whether it belongs to the program in the database and suggest the top-k programs. 
Given the event data during a time window $U = \{e_1,e_2,...,e_n\}$ of a target program with a claimed name/ID, we check whether it belongs to the claimed program. If it matches the behavior pattern of the claimed program, the predicted label should be +1, otherwise it should be -1. Slightly more formally,  %we formulate it as a binary classification problem: 
given event data $E$ of a program, a mapping function $f$ is used to map $E$ to a binary label $Y\in \{+1,-1\}$, such that $f:U\rightarrow \{+1,-1\}$.%Due to the unique characteristic of the program event data, we propose attentional multi-channel graph neural network to model this mapping function.
%\myred{Briefly point out the differences between our work and malware detection}
\nop{
Our formulated problem is related to malware detection, but is different from that in four folds: 
(1) Malware detection focus on the malicious program and needs large amounts of labeled malware samples to train the model, which is difficult to obtained. Different from that, program verification pays attentions on the benign programs and does not require malware samples,
(2) Program verification is the step prior to the malware detection, which focuses on detecting whether the program name is disguised.
(3) Malware detection usually relies on the program signature, which can be evaded by changing the signature using code obfuscation or repackaging.
(4) Malware detection highly depends on the expert knowledge. Different from that, program verification is expert knowledge free and performed in a data driven way. 
}

% TODO: If the program with a brand-new exename, we assume it would be easily caught. 

% \subsection{Challenge}
% However our problem is very challenging. The main challenges come from unique characteristic of the system surveillance data, which is as followed:
% \begin{itemize}
% \item High Volume: System events can be generated at a high frequency (e.g., tens of thousands events per second). In a modern computer system, plentiful system events can take place “silently” in the backstage without users ever being aware of them. It results tens thousands of program events within a machine in a day.
% \item High Heterogeneity: There are multiple type of program events(P-P, P-F, P-I) and multiple type of system entities(Process, File, Internet Socket).
% \item High Dynamic: The behavior of the same program changes over time and/or machine. Different versions of the same program can behave slight different.
% \item Rich Categorical Attributes: The attributes in source and destination entity are all categorical. However, due to the lack of an intrinsic proximity measure, many powerful algorithms for numerical data analysis may not work well on their categorical counterparts, making it a bottleneck in practical applications.
% % \item High Uncertainty: There are more than thousand of program in a machine, which causes high uncertainty 
% \end{itemize}

% 1.       Rule1:  One idea per paragraph.

% 2.       Rule2: First sentence of the paragraph gives the gist summary of what the paragraph is about. The rest of the paragraph is a more detailed explanation of the idea.

% 3.       Rule 3:  The first sentence of each paragraph should tell the story/key points and logical structure of the paper should become apparent.

% 4.       Rule4: Each sentence should be no longer than two lines.

% 5.       Rule 5: Each paragraph should be no longer than a quarter of a page.

% 6.       Rule6:  Two subsequent sentences must be logically linked via a pair of key phrases, one in each sentence.

% 7.       Rule7: Always define the big picture first (umbrella speech)  before going into details of the individual pieces and components.

% 8.       Rule8:  The headings of the sections/subsections must be content rich. It must be a punch line summary of the entire section/subsection.

% 9.       Rule9: The title of the paper should have the problem being addressed in the paper, the technology being used to solve the problem and the impact.

% 10.   Rule10: The technology should be specific whereas the impact more generic.

% Example: ``A novel method for crosstalk prediction''

% This is a very badly phrased title and has the following flaws:

% 1)      Never use the word "novel" in the title.

% 2)      The type of method is too vague.

% 3)      The impact is absent.

% A   better title would be " A statistically robust and accurate method for metabolic pathway crosstalk discovery via bayesian driven information fusion"

% 11.   Rule 11: Every word in the title must be explained in the introduction.

% 12.   Rule 12: A clear paragraph of the major contribution and innovations must be listed.

% 13.   Rule 13: For each novelty claim there must be a clear parallel in the results section with scientific evidence supporting that claim(do not make speculative claim that cannot backed up by evidence).

% 14.   Rule 14: Do not provide a laundry list of problems/limitations with existing methods, instead you may complement existing methodologies and state clearly how your work is complementary to the existing methodologies.

% 15.   Rule 15: Make sure that the limitations that you mention are in fact the ones that your method addresses. If their limitations are presented as state of the art in the field then the paper must be specific about which particular limitation from that list the paper addresses.  You must give an intuition about the underlying trick in the methodology that indeed helps to address the problem.

% 16.   Rule 16:  The introduction section must be self contained. It is a marketing speech that helps you sell your paper. Each paragraph has to have all the key elements. The motivation, specific technical problem addressed , why it is technically challenging, what approaches have been proposed to address the problem, what specific limitations of the existing approaches that your paper addressed, how it fixes the limitation and the summary of the results that lets the reader's conclude that the issues that have been addressed.

% 17.   Rule 17: Keep in mind that busy people do not read beyond introduction.

% 18.   Rule 18: Less first personal words and passive sentences, e.g., In table 1, X is presented ... --> Table 1 presents X ...; Our methods are compared to --> the proposed methods are compared to ...

% 19.   Rule 19: Break long sentence to several short sentences;

% 20.   Rule 20: Provide two tables if possible, table 1 in the end of problem  definition, gives all the symbols used in the paper, table 2 in the  beginning of experiment section, gives all the parameter setting and

% datasets description in the experiments;


==> bk/03-method.tex <==
\section{Algorithm}

\begin{figure*}[htb]
\centering
\vspace{-10pt}
\includegraphics[width = 1\linewidth]{fig/general_framework_binary_6.pdf}
\caption{System Architecture of \ours}
\label{fig:Architecture}
\vspace{-15pt}
\end{figure*}
%\myred{TODO: The method is too long. will cut at least 0.5-1 page, especially the behavior graph modeling subsection}
\subsection{Overview}
In this section, we introduce \ourss, a graph neural network based approach to verify the system program in a data-driven manner. The framework of \ourss\ (as shown in Figure \ref{fig:Architecture}), consists of the following six components:
\begin{itemize}
\vspace{-2pt}
\item \textbf{Surveillance Data Collection}
%The low-level system events are collected from a enterprise network. 
This module collects three different types of low-level system events (see Section \ref{sec:pre} for definition) from IT/OT systems. %including a process folks another process (P$\rightarrow$P), a process access a file (P$\rightarrow$F), and a process connects to INETSocket (P$\rightarrow$I) across three types of system entities.
%Three type of system entities are considered, including process, file and INETSocket.
\vspace{-10pt}
\item \textbf{Behavior Graph Modeling}
Based on the collected program event data, a compact heterogeneous program behavior graph is constructed for the target process from large-scale program event data to capture the complex interactions and eliminate the data redundancies.
%Since the raw attribute of each entity are extreme high dimensional and categorical, which are difficult to use without any expert knowledge, we extract the knowledge-free feature for each entity.  
\vspace{-8pt}
\item \textbf{Multi-Channel Transformation}
This module transforms the generated heterogeneous behavior graph to multi-channel graphs with each channel modeling one type of meta-path relationship. 
%The knowledge-free feature are extracted for each entity within each channel graph.  
\vspace{-8pt}
\item \textbf{Contextual Graph Encoder}
Based on the generated multi-channel graph, we propose an effective graph neural network with propagation layer and perceptron layer to extract the graph embedding. %from the target process context. 
%the directed graph embedding. Benefit from flexible context propagation, we can capture the directed causal relation.
\vspace{-8pt}
\item \textbf{Channel-Aware Attention}
In this module, an attention mechanism is proposed to align the graph embeddings extracted from different channels and generate the attentional joint embedding.

\vspace{-8pt}
\item \textbf{Program Reidentification}
After the joint embedding is extracted, the generated  low-dimensional vector 
%of program behavior data 
is fed to a classification layer to generate the prediction. %Specifically, we use logistic regression at classification layer.   
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Specifically, given a program system event snapshot, we first perform the \emph{Behavior Graph Modeling} and construct a heterogeneous graph to reduce the data redundancy and capture the complex interaction among system entities.
% % In this section, we formally propose \ours, a deep learning based approach to learn the representation of the program behavior in a data-driven manner. The framework of \ours is shown in Figure \ref{fig:GF}. Specifically, given a program system event snapshot, we first perform the \emph{Behavior Graph Modeling} and construct a heterogeneous graph to reduce the data redundancy and capture the complex interaction among system entities.
% %(see Section ??). 
% Then we perform \emph{Multi-Resolution Augmentation} to 
% capture the dynamic of the constructed graph
% %enhance the dynamic robustness of the constructed graph.
% %preserve the dynamic property of the constructed graph.
% %(see Section ??) 
% Next, the \emph{Multi-Channel Transformation} is proposed to transform the heterogeneous graph to the Multi-Channel homogeneous graph.
% %(see Section ??) 
% After that, we proposed \emph{Contextual Graph Encoder}
% %\emph{Contextual Directed Graph Encoder}
% , a new graph neural network to extract the representation of the graph for each channel.
% %(see Section ??) 
% When the representation of each channel graph is obtained, we introduce \emph{Channel-Awareness Attention}, an attention mechanisms, to align the learned representations from different channels and generate the joint representation. Finally, we perform \emph{Contrastive Analysis Objective} to learn the parameter of the proposed model. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5



%Since each system event, models the directed dependency from a process to another system entity, the constructed program behavior graph is a directed graph. Moreover, the involved system entities and their directed dependencies are heterogeneous. The resulted program behavior graph is also heterogeneous. After the program behavior graph is constructed, we propose a deep graph representation learning approach to to learn the graph embedding(see Section ??). However learning from a directed graph with high heterogeneous, high dynamic is very challenges. To overcome these challenges, we propose a novel deep learning architecture, Multi-View Multi-Resolution Directed Graph Encoder, namely \ours. It consists of a number novel components, including Multi-Resolution Augmentation, Multi-View Modeling, Contextual Directed Graph Encoding and View Attention. The Multi-Resolution Augmentation track down the problem of the high dynamic. We use Multi-View Modeling to capture the high heterogeneity. To learn good feature representation from directed graph, a Contextual Directed Graph Encoding is proposed. To further reinforce the Multi-View modeling, we propose the View-Aware Attention. We perform contrastive analysis to train our mode. When the graph embedding is obtained, we can use it for different tasks, such as disguised program detection, Malware detection and version upgrade detection. 
% In the following sections, we discuss the details of each components.
% In this section, we formally propose Deep Program Re-ID, a deep learning based approach to learn to re-identify the program in a data-driven manner. The framework of Deep Program RE-ID is shown in Figure \ref{fig:GF}. Specifically, given the program system event data, we first construct the program behavior graph that capture the complex interaction among system entity (see Section ??). Since each system event, models the directed dependency from a process to another system entity, the constructed program behavior graph is a directed graph. Moreover, the involved system entities and their directed dependencies are heterogeneous. The resulted program behavior graph is also heterogeneous. After the program behavior graph is constructed, we propose a deep graph representation learning approach to to learn the graph embedding(see Section ??). However learning from a directed graph with high heterogeneous, high dynamic is very challenges. To overcome these challenges, we propose a novel deep learning architecture, Multi-View Multi-Resolution Directed Graph Encoder, namely \ours. It consists of a number novel components, including Multi-Resolution Augmentation, Multi-View Modeling, Contextual Directed Graph Encoding and View Attention. The Multi-Resolution Augmentation track down the problem of the high dynamic. We use Multi-View Modeling to capture the high heterogeneity. To learn good feature representation from directed graph, a Contextual Directed Graph Encoding is proposed. To further reinforce the Multi-View modeling, we propose the View-Aware Attention. We perform contrastive analysis to train our mode. When the graph embedding is obtained, we can use it for different tasks, such as disguised program detection, Malware detection and version upgrade detection. 
% In the following sections, we discuss the details of each components.



\subsection{Behavior Graph Modeling}
\label{subsec:graph}
%When a program is executed in the operation system, we can produce system events data by monitoring the behavior of the program. By observing and analyzing the system event data, we found that they has four properties: 
Real information networks like the enterprise networks often generate a large volume of system behavioral data with rich information on program/process level events. We utilize a system monitoring tool based the Windows ETW~\cite{etw} \nop{} and Linux audit framework~\cite{kernelaudit}} to collect the program behavioral event data. The data has four properties:
(1) High Volume. The system event data collected from a single computer system 
%by monitoring the process interactions 
in one day can easily reach 20 GB and the number of events relate to one specific program can easily reach one million. It is prohibitively expensive to perform analytic task on such massive data in terms of both time and space. 
(2) High Dimension. Each system event is associate with thousands of attributes, including information of involved system entities and their relationship. This causes the curse of dimensionality \cite{verleysen2005curse}. 
(3) Categorical. 
All available attributes are categorical and each attribute has large amount of categories. 
%For example, in a single computer system, the number of the filename and the number of IP address accessed within one week can easily reach 10k. 
Analysis on categorical data is very challenging due to the lack of intrinsic proximity measure \cite{boriah2008similarity}. 
(4) Redundant. 
The attributes are redundant. 
Most of the attributes of system entities are same. Repeatedly saving these attributes results a significant redundancy. The events are also redundant. The event with same system entity and relationship are usually repeatedly stored, which also causes a notable redundancy.
These motivate our idea of graph modeling.  
%Therefore, we devise a compact graph representation of the system event data.
%By observing and analyzing the system event data, we found that they are usually redundant. The redundancy comes from several sources. 
%Firstly, the attributes are redundant. Most of the attributes of system entities are same. Repeatedly saving these attributes results a significant redundancy.   
%Furthermore, the events are redundant. The event with same system entity and relationship are usually repeatedly stored, which also causes a notable redundancy. These redundancy motivates our idea of graph modeling. 

We construct the compact graph to modeling the program behavior. Formally, given the program event data $D$ across several machines within a time window, a heterogeneous information network $G = (V,E)$ is constructed for the target program. $V$ denotes a set of vertices, each represents an entity, belongs to three types: process (P), file (F), INETSockets (I), namely $V = P \cup F \cup I$. The number of entity is $n_v$. $E$ denotes a set of edges(dependency) $(v_s,v_d, r)$ between the source entity $v_s$ and destination entity $v_d$ with relation $r$. We consider three types of relations, including: (1) a process forking another process (P$\rightarrow$P), (2) a process accessing a file (P$\rightarrow$F), and (3) a process connecting to an Internet socket (P$\rightarrow$I). Each graph is associated with an adjacency matrix $A$. 
%Since the constructed graph is directed, $(v_s,v_d, r) \neq (v_d,v_s, r)$. 
With the help of the behavior graph modeling, data redundancy is significantly reduced but rich information are still kept. 
%With the help of the behavior graph modeling and entity feature extraction, we can reduce the data redundancy significantly but still keep rich information. 

%but preserve the heterogeneous dependency between heterogeneous system entities to capture the program behavior.

% We cast polypharmacy side effect modeling as a multirelational link
% prediction problem on a multimodal graph encoding drug, protein, and
% side effect relationships (Figure 1). More precisely, these relationships are
% represented by a graph G = (V, R) with N nodes (e.g., proteins, drugs)
% vi ∈ V and labeled edges (relations) (vi, r, vj ), where r is the edge type
% (relation type): (1) physical binding between two proteins, (2) a target
% relationship between a drug and a protein, or (3) a particular type of a
% side effect between two drugs. As mentioned in Section 2 we consider 964
% different relation types between drugs (i.e., side effects).
% In addition, we allow for inclusion of side information in the form
% of additional node features. Different nodes (drugs, proteins) can have
% different number of node features, given by real-valued feature vectors
% x1, x2, . . . , xN assigned to every node in the grap

% In this paper, we are interested in only those event sequences
% that happen in a given time interval, namely the timespan is less
% than or equal to ∆t, where ∆t is a given threshold. Figure 2 shows
% an example of the compact graph for enterprise surveillance data.
% Note that according to the types of interactions that are allowed in
% UNIX, G is not a complete graph. Instead, it only allows the edges
% between (1) process and file nodes, (2) process and process nodes,
% (3) process and socket (both UDSockets and INETSockets) nodes,
% and (4) UDSocket and UDSocket nodes.
% By removing the redundancy of attributes and events, our graph
% representation can significantly compress the original heterogeneous
% event data while preserving relevant information for intrusion
% detection. Our experiment results in Section 4 demonstrate
% that the graph model reduces the space cost significantly.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Multi-Resolution Augmentation}
% % dynamic nature of the system event data
% Due to the dynamic of the computer system, the behavior of the program can changes over time and/or machine. Different versions of the same program can behave slight different. For instance, a program's behavior can be very active during the weekday but relevant salient during the weekend. Another example is that, a researcher may only use ACROBAT.exe for document view, while a staff may use it for both document view and edit. The program's behavior can vary depend on the user's behavior. This kind of dynamic affect the structure of the constructed behavior graph. There it is required that the constructed graph should capture the intrinsic dynamic propriety. 

% The idea of the Multi-Resolution Augmentation is motivated by multi-resolution data augmentation in computer vision. 
% %In the real world scenario, we may have a data of program collect in a limited set of conditions. But, our target program may exist in a variety of conditions.
% We account for dynamics by aggregating the program behavior graphs spatially and temporally in order to consider the graph data in different resolutions. Formally, we consider the raw program behavior graph as resolution-1 graph in both time and agent, which is defined as $\mathcal{G}^{1,1}$, with the superscript denoted the resolution in the space and time. They are the most basic element to construct higher resolution graph. To get the higher resolution graph, we perform an concatenation function on the resolution-1 graph, such that
% \begin{equation}
% \mathcal{G}^{r_a,r_t}=CAT_{r_a,r_t}(\mathcal{G}^{1,1})
% \end{equation}
% where $CAT$ is a graph concatenation function. It has two parameters $r_a$ and $r_t$, which is denoted as the resolution number in space and time respectively. Specifically, we constructed the new graph with all entities exit in the resolution-1 graph and place an directed edge between two entities without duplication. We use these higher resolution graph sets to augment the original data in order to capture the dynamic uncertainty of the program. 
% % can be theoretical 
% % 1--cover the uncertainty in the data
% % 2--cover the adversal sample
% % 3--cover the https://pdfs.semanticscholar.org/4cc1/849707bc139b877b5985d9e82ba5c9306f7c.pdf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Attentional Multi-channel Graph Neural Networks}
\label{subsec:att}
After the behavior graph modeling, a heterogeneous program behavior is obtained. There exist a hierarchy of different dependencies from simple to complex. Among all the dependencies, the complex ones are not exposed directly by the edge in the graph, but can be inferred by a hierarchy of deep representation. For example, a process accessing a file (P$\rightarrow$F) is a simple dependency, two processes  accessing the same file (P$\rightarrow$F$\leftarrow$P) is a complex dependency. The complex dependency can not be modeled directly with shallow representation such as simple dependency, but can be inferred from a hierarchy of deep representation, from simple dependency (P$\rightarrow$F) to (P$\rightarrow$F$\leftarrow$P). To infer the relationship of two processes accessing the same file, we can check whether they share the same context. Due to the complex and obscure dependency, it requires a deep graph structure learning model to capture the hierarchical dependency. However, recent deep graph structure learning methods \cite{kipf2016semi,defferrard2016convolutional,bruna2013spectral,hamilton2017inductive,velickovic2017graph} only work for homogeneous undirected graph and can not capture the heterogeneity of HIN.
%There are multiple type of entities and multiple type of connections. The diversity among different entities and edges are large. 
To learn hierarchical dependency representation (hierarchical graph embedding) from HIN, we design attentional multi-channel graph neural network, which consists of multi-channel transformation, input layer, contextual graph encoder and channel-aware attention. Here, we introduce these components one by one and build the model step by step. 

\noindent{\bf{Multi-channel Transformation}}
To make HIN learnable via a deep representation learning, we design a multi-channel transformation module to transform the heterogeneous graph to multiple channels of homogeneous graphs guided by the meta-paths.
%significantly increases the difficulty to learn the representation of heterogeneous graph. Recently graph neural networks (GNNs) methods \cite{kipf2016semi,defferrard2016convolutional,bruna2013spectral,hamilton2017inductive,velickovic2017graph} is becoming more and more popular due to their powerful representation learning ability on graph. However these methods can only applied to homogeneous graph. To address the problem of learning representation from heterogeneous graph, we introduce the multi-channel transformation module to transform the heterogeneous graph to multiple channels of homogeneous graphs guided by the meta-path.
%The multi-channel transformation is a two-stage transformation: (1) it transform the heterogeneous graph to homogeneous, (2) it transform the homogeneous directed graph to homogeneous undirected graph. 
A meta-path \cite{sun2011pathsim} is a path that connects entity types via a sequence of relations over a heterogeneous network. For example, in a computer system, a meta-path can be the system events (P$\rightarrow$P, P$\rightarrow$F, P$\rightarrow$I) described in Section 2, with each one defines a unique relation between two entities.
%and can be used as the link in a specific channel in the multi-channel graph. 
\nop{
(1) relationship of a process forking another process (P $\rightarrow$ P),
(2) relationship of a process accessing a file (P $\rightarrow$ F),
(3) relationship of a process opening an Internet socket (P $\rightarrow$ I),
(4) relationship of two processes accessing the same file (P $\rightarrow$ F $\leftarrow$ P), 
(5) relationship of two processes opening the same Internet socket (P $\rightarrow$ I $\leftarrow$ P).} 
%Specifically, we model the inbound neighborhoods and outbound neighborhoods separately in different channels for each type of directed connection.    
To model the heterogeneous dependency, we transform the heterogeneous graph into multi-channel graph with each channel graph connected via a certain type of meta-paths. Formally, given a heterogeneous graph $\mathcal{G}$ with a set of meta-paths $P=\{P_1, ... ,P_{|C|}\}$, the translated multi-channel network $\hat{G}$ is defined as:
\vspace{-5pt}
\begin{equation}
\hat{G}=\{G_i | G_i=(V_i,E_i, A_i) , i=1,2,...,|C|) \}
\end{equation}

where $E_i$ denotes the homogeneous links between the entities in $V_i$, which are connected through the meta-path $P_i$. Each channel graph $G_i$ is associated with an adjacency matrix $A_c$. $|C|$ denotes number of meta-paths.
%Since we consider six types of meta-path in computer system, we transform the program behavior graph into a 6-channel graph.
\nop{
For each entity in each channel graph, there exists high-dimensional attributes, which are difficult to extract feature without any expert knowledge. Hand feature engineering is time-consuming and the quality of the feature are not guaranteed. To address these problems, we extract the knowledge-free feature for each entity. Based on context of the entity, we extract two type of features: connectivity feature and graph statistics feature. 

\begin{itemize}
\item \textbf{Connectivity Feature}
Connectivity feature are constructed to describe the pairwise proximity between entities. It is defined as $X^{con}_{v}=\{\hat{e}_{v, 1}...,\hat{e}_{v, |V|}\}$, which denotes the first-order proximity between $v_u$ and other entities. 

\item \textbf{Graph Statistic Feature}
Graph statistics feature are generated based on the graph theory. It is defined as $X^{stat}_{v}=\{X_v^{s1},X_v^{s2},X_v^{s3},X_v^{s4}\}$, including four graph measurements, including degree centrality, closeness centrality, betweenness centrality and clustering coefficient. 
The degree centrality is defined as the number of links incident upon an entity. The degree can be interpreted in terms of the immediate risk of an entity for catching whatever is flowing through the network (such as a virus, or some information).  
The closeness centrality is the average length of the shortest path between the entity and all other entities in the graph. Thus the more central an entities is, the closer it is to all other entities.
The betweenness centrality quantifies the number of times an entity acts as a bridge along the shortest path between two other entities. It was introduced as a measure for quantifying the control of an entity on the communication between other entities in the graph. In this conception, entity that have a high probability to occur on a randomly chosen shortest path between two randomly chosen entities have a high betweenness.
The clustering coefficient measures the degree to which entities in a graph tend to cluster together. It characterizes a higher-order proximity of a pair of entities, even if they are directly connected. Therefore it can capture the global structure and robust to sparse structure.   
\end{itemize}
\nop{\myred{maybe some more detail about feature extraction}}
}

\noindent{\bf{Input Layer}}
After the multi-channel transformation, an input layer is applied to construct the feature vector for each entity. Specifically, two types of features are constructed: connectivity feature and statistic feature. Since these features are constructed without any expert knowledge, they are knowledge free. 

Connectivity features are constructed to describe the pairwise proximity between entities. It is defined as $X^{con}_{v}=\{e_{v, 1}...,e_{v, |V|}\}$, which denotes the first-order proximity between $v_u$ and other entities. Graph statistical features are generated based on the graph theory. It is defined as $X^{stat}_{v}=\{X_v^{s1},X_v^{s2},X_v^{s3},X_v^{s4}\}$, including four graph measurements: degree centrality, closeness centrality, betweenness centrality, and clustering coefficient.

\noindent{\bf{Contextual Graph Encoder}}
In this step, we feed the multi-channel graph and the corresponding entity feature to a graph neural network for graph embedding. To learn the hierarchical graph representation, we propose contextual graph encoder (CGE) and stack a deep graph neural works.
%In this section we introduce the proposed novel GNNs Model, named Contextual Graph Encoder (CGE) in order to learn deep graph representation from each channel of homogeneous directed graph. 
Given the homogeneous graph $G = (V, E, A)$ with each $V$ associated with a corresponding feature $X$, our target is to learn an encoding function $f_{G}:G \rightarrow h_{G}$, that encodes the graph to a low dimensional vector (graph embedding). $h_{G}$ denotes the generated graph embedding vector. Specifically, we use the representation of the target entity $h_{v_{t}}$ (target contextual entity embedding) which encodes both contextual structure and its own features by a mapping function $f_{V}:V \rightarrow h_{V}$ as the representation of the graph. In this way, we reduce the graph embedding problem into target entity embedding. Formally, our graph encoder is defined as follows:
\begin{equation}
h_{G} = h_{v_{t}} = f_{V}(V_t)
\end{equation}
\vspace{-5pt}

The basic contextual graph encoder consists of a propagation layer $PROP()$ and a perceptron layer $PERCE()$. The propagating layer propagates the information from the context of the target entity. We defines the propagation layer $PROP()$ as follows:
\begin{equation}
\hat{h}^l=PROP(h^l)=P^lh^l
\end{equation}
\vspace{-5pt}

where $l$ denotes the layer number, $P^l$ denotes the propagation matrix at layer $l$ and 
$\hat{h}^{l}$ indicate the output of $PROP()$ at layer $l$. The first layer $h^0=X$ takes the feature of each entity. 
The propagation layer propagates information to the target entity within a region, named graph receptive field $\mathcal{F}$. The graph receptive field $\mathcal{F}$ usually consists of all L-hop contexts of target entities. The propagation operation encodes both graph structure and the entity features, which is similar to performing a graph convolution operation \cite{kipf2016semi}. After the propagation is performed, a perceptron layer $PERCE()$ is applied to the propagated representation of the entities, such that:
\begin{equation}
h^{l+1}=PERCE(\hat{h}^l)=\sigma(\hat{h}^lW^l)
\end{equation}
where $W^l$ is the shared trainable weight matrix for all the entities at layer $l$ and $\sigma()$ is a nonlinear gating function. Benefit from weight sharing, it is both statistically and computational efficient compared with traditional entity embedding. Weight sharing can act as powerful regularization to preserve the invariant property in the graph and the number of parameters are significantly reduced.

\nop{
Based on the definition of $PROP()$ and $PERCE()$, graph encoder has different variations. The propagation matrix can be defined in several ways. In the simplest case, $P=I$, with $I$ denotes the identity matrix. The encoder is exactly a multi-layer perceptron (MLP),such that 
\begin{equation}
\hat{h}^l=PROP(h^l)= I h^l = h^l
\end{equation}
The graph receptive field is defined as $F=\{v_t\}$, without considering any context.

The propagation can be performed via diffusion process characterized by a random walk on the graph with a specific probability $q \in [0,1]$ and a state transition matrix $D^{-1}A$. Here $D$ denotes the degree matrix of the adjacency matrix $A$, such that $D=diag(A \textbf{1})$. \textbf{1} is a all one vector. After a number of transitions, such markov process converges to a stationary distribution $P\in\mathcal{R}^{N \times N}$ with $i$th row indicates the likelihood of diffusion from entity, hence the proximity of that entity. This stationary distribution of the diffusion process are proven to have a closed from solution. When consider the 1-step truncation of the diffusion process, the propagation layer is defined as followed:
\begin{equation}
\hat{h}^l=PROP(h^l)=D^{-1}Ah^l=\sum_{u\in N(v_t)}P_{uv_t}h^l
\end{equation}
The receptive field is defined as $F=\{N(v_t)\}$, with $N(v_t)$ denotes all context of target entity $v_t$. The propagation layer computes weighted sum of the context's current representation. This is closely related to diffusion convolution \cite{atwood2016diffusion}.

The propagation can also be considered in a spectral space as GCN \cite{kipf2016semi}. In this case, the propagation layer is defined as followed:  
\begin{equation}\label{eq:prop}
\hat{h}^l=PROP(h^l)= \hat{D}^{-1/2} \hat{A} \hat{D}^{-1/2} h^l
\end{equation}

where $\hat{A}=A+I$ denotes the normalized adjacency matrix and $\hat{D}=diag(\hat{A} \textbf{1})$ denotes the normalized degree matrix. The graph receptive field $F=\{N(v_t)\}$ is exactly the same as random walk propagation.

The previous methods leverage full set of context to define the graph receptive field, which is computational expensive. To reduce the size of receptive field, context sampling can be adopted as \cite{hamilton2017inductive}. The context can be sampled with a uniform sample distribution, such that
\begin{equation}
P h^l \approx \frac{n(v)}{|n^l(v_t)|} \sum_{u \in \hat{n}^l(v_t)} P_{uv_t} h^l = \hat{P} h^l
\end{equation}
where $n(v_t)$ is the set of random sampled context and $\hat{n}(v_t)$ is the subset of it, which denotes the sampled context for layer $l$. Random context sampling reduces the graph receptive field size from all the L-hop neighbors to $\sum_{l=1}^L |\hat{n}(v_t)|$. This is equivalent to replace the original propagation matrix $P$ with a sparser unbiased estimator $\hat{P}$, such that $E \hat{P}^l=P$, where $ \hat{P}^l_{uv_t}=\frac{n(v_t)}{|n^l(v_t)|} P_{uv_t}$ if $u \in n^l(v_t)$. 
}

%In this work, de defined the receptive field as \myred{as what ???}\cite{hamilton2017inductive}.

%The context is sampled with a uniform sample distribution, such that
\nop{
By sampling the context with a uniform distribution \cite{hamilton2017inductive}, we can define the propagation matrix as follows: 
\begin{equation}
P^l \approx \frac{n(v_t)}{|\hat{n}^l(v_t)|} \sum_{u \in \hat{n}^l(v_t)} P^{l}_{(v_t, u)} = \hat{P}^{l}
\end{equation}
where $n(v_t)$ indicates the contexts of the target entity $v_t$ and $\hat{n}^l(v_t)$ indicates the sampled contexts at layer $l$, with $\hat{n}^l(v_t)\subset n(v_t)$. $P^{l}_{(v_t, u)}$ denotes the propagation from entity $u$ to entity $v_t$. 

the set of the sampled context and $\hat{n}(v_t)$ is the subset of it. 
%which denotes the sampled context for layer $l$. 
The corresponding graph receptive field at layer l is defined as $\mathcal{F}=\{\hat{n}^l(v_t)\}$. Random context sampling reduces the size of graph receptive field from all the L-hop neighbors to $\sum_{l=1}^L |\hat{n}^l(v_t)|$. 
In this way, we use a sparser unbiased  $\hat{P}$, such that $E \hat{P}^l=P$, where $\hat{P}^l_{uv_t}=\frac{n(v_t)}{|n^l(v_t)|} P_{uv_t}$ if $u \in n^l(v_t)$, where these stochastic contexts and build a three layer CGE in the following way:  
}
We design our propagation layer by performing random walk on the graph via diffusion process characterized by a specific probability $q \in [0,1]$ and a state transition matrix $D^{-1}A$. Here $D$ denotes the degree matrix of the adjacency matrix $A$, such that $D=diag(A \textbf{1})$. \textbf{1} is a all one vector. After a number of transitions, such markov process converges to a stationary distribution $P\in\mathcal{R}^{N \times N}$ with $i$th row indicates the likelihood of diffusion from entity, hence the proximity of that entity. This stationary distribution of the diffusion process are proven to have a closed form solution \cite{atwood2016diffusion}. When consider the 1-step truncation of the diffusion process, the propagation layer is defined as followed:
\begin{equation}
\hat{h}^l=PROP(h^l)=D^{-1}Ah^l=\sum_{u\in N(v_t)}P_{uv_t}h^l
\end{equation}
The receptive field is defined as $\mathcal{F}=\{N(v_t)\}$, with $N(v_t)$ denoting all the contexts of target entity $v_t$. The propagation layer computes weighted sum of the contexts' current representation. In this way, we build a three layer CGE as follows:
%This is equivalent to replace the original propagation matrix $P$ with a sparser unbiased estimator $\hat{P}$,  $E$ is the sparser unbiased estimator such that $E (P) = \hat{P}^l$, where $\hat{P}^l_{uv_t}=\frac{n(v_t)}{|n^l(v_t)|} P_{uv_t}$ if $u \in n^l(v_t)$. we propagating over
\vspace{-0.5em}
\begin{align}
h^1 = \text{ReLU}((P^0 X) W^0)\\
h^2 = \text{ReLU}((P^1 h^1) W^1)\\
h^3 = \text{ReLU}((P^2 h^2) W^2)\\
h_{G} = h_{v_{t}} = h^3
\label{eq:sp}
\vspace{-0.5em}
\end{align}
where $\text{RELU}()$ is a element-wise rectified linear activation. We perform the CGE to each channel graph and generate corresponding graph representation respectively.
\nop{
The proposed CGE can applied to both undirected and directed graph. To capture the directed dependency, we consider diffusion process in two directions to capture the influence from both inbound neighbourhood and outbound neighbourhood. In this case, the propagation layer is defined as followed:
\begin{equation}
\hat{h^l}=PROP(h^l)=(\beta_1 D_{O}^{-1} A + \beta_2 D_{I}^{-1} A^T) h^l
\end{equation}
where $D_{O}^{-1}$ indicates the out-degree diagonal matrix, $D_{I}^{-1}$ indicates the in-degree diagonal matrix and $\beta_1, \beta_2$ are the weight of them.
}
%importance sampling 

%To learn the representation of entity $\mathcal{H}_v_{t}$ 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Contextual Graph Neural Encoder-general version}
% In this part, we adopt the neighborhood encoding approach as in \cite{hamilton2017inductive} for aggregating information from local neighborhoods. It consists of three main steps: (1) neighborhood sampling; (2) neighborhood aggregation; (3) feature concatenation. By iterating over these three steps recursively, node embeddings can be updated to encode more and more structural information. We define $K$ to be the depth of the neighborhood search. To propagate information in the depth of $K$, $K$ aggregation functions are required. Each aggregation function can be defined as $f_{agg}^k$ with corresponding parameters $\mathbf{W}^k, \forall k \in [1, K]$. The three main steps of neighborhood encoding are described as follows.

% %To propagate information between $K$ layers of model or search in $K$ steps, $K$ aggregation function can be used. Each aggregation function can be defined as $\text{AGG}_k, \forall k \in [1,K]$ with corresponding weight matrices $\mathbf{W}^k, \forall k \in [1, K]$. 
% %During the encoding phase, the node embedding are initialized to be equal to the node's attributes. 
% %Then at each iteration of the encoder algorithm, node aggregate the embedding of their neighbors, using an aggregation function that operates over sets of vectors. After this aggregation, every node is assign 
% %Then at each iteration of the neighborhood encoding consists of three basic steps: 1.neighborhood sampling; 2.neighborhood aggregation; 3.Feature concatenation.

% \subsubsection{Neighborhood Sampling}
% For each node $v \in \mathcal{V}$, a fixed-size neighborhoods are sampled uniformly. Formally, we define the neighborhood as a set of nodes $\{u \in \mathcal{V} :(u,v) \in \mathcal{E}\}$. The sequence of sampled fixed-size nodes is defined as $\mathcal{N}^k (v)$, and the sample size is defined as $S_k, \forall k \in [1, K]$. When the node degree is less than the neighbor sample size, we randomly select the neighbors with replacement until the desired sample size is met.

% %A sequence of fixed-sized nodes $\mathcal{N}(v)$ is drawn uniformly from the set $u \in \mathcal{V} :(u,v) \in \varepsilon$. 

% \subsubsection{Neighborhood Aggregation}
% We aggregate the representations of the nodes in the sampled sequence $\mathcal{N}^k (v)$ into a single vector representation $\mathbf{h}^{k-1}_{\mathcal{N}(v)}$ via the aggregation function $f_{agg}^k$. During the neighborhood aggregation procedure, the representation of a node is the node embedding generated from the previous neighborhood encoding $\mathbf{h}^{k-1}_{u}, \forall u \in \mathcal{N}(v)$. The initial node representations are input features.

% %is aggregate the attributes of its immediate neighborhood $h^{k-1}_{u}, \forall u \in \mathcal{N}(v)$ into a single vector $h^{k-1}_{\mathcal{N}(v)}$. The aggregation depends on the representations of the node embedding generated at the previous step. At the beginning the node embbedding are initialized to be equal to the node's attributes.

% \subsubsection{Feature Concatenation.}
% In this step, the current representation $\mathbf{h}_v^{k-1}$ is augmented with the aggregated neighborhood vector $\mathbf{h}^{k-1}_{\mathcal{N}(v)}$. The concatenated representation is then fed to a fully connected neural network which generates a new representation of the node. In the end, the final representation of the node is denoted as $\mathbf{z}_v \equiv \mathbf{h}^K_v$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent{\bf{Channel-Aware Attention}}
Going through the CGE, the graph embeddings for each channel graph are extracted. However, the different channels should not be considered equal. For example, Ransomware is usually very active in accessing the files but barely folks a process or opens a internet socket while the VPN is usually very active in opening the internet socket but it barely accesses a file or folks a process. Therefore, we need to treat different channels differently. In this part, we propose channel-aware attention, an attention mechanisms, to align the graph embeddings from different channels and generate the joint embedding. Specifically, we learn the attention weights for different channels automatically.

Formally, given the corresponding graph embedding $h_{G_c}$ for each channel $c=1,2,...,C$, we define the attention weight as followed:
\vspace{-5pt}
\begin{equation}
\alpha_{c}=\frac{\exp (\sigma(a[W_a h_{G_c}||W_a h_{G_k}]))}{\sum_{k'\in C} \exp (\sigma (a[W_a h_{G_c}||W_a h_{G_{k'}}]))}
\label{eq:att}
\end{equation}
where $h_{G_c}$ is graph embedding of the target channel, $h_{G_k}$ denotes the representation of the other channels. $a$ denotes a trainable attention vector, $W_a$ denotes a trainable weight mapping the input features to the hidden space, $||$ denotes the concatenation operation and $\sigma$ denotes the nonlinear gating function. We formulate a feed-forward neural networks that is used to compute the correlation between target channel and the other channels. This correlation is normalized by a softmax function. Let $\test{ATT}(h_{G_c})$ represent Eq.(\ref{eq:att}). The joint representation of each channel can be represented as followed:
\begin{equation}
h_{G_{Join}}=\sum_{c=1}^{C} \test{ATT}(h_{G_c}) h_{G_c}
\end{equation}
\vspace{-5pt}

The channel-aware attention allow us to better infer the importance of different channels by leveraging their correlations and learn a channel-aware representation. 
%In this way, we can mode the different type of program system level behavior differently. 
\vspace{-5pt}
\subsection{Program Reidentification}
After the joint graph embedding is generated from program event data, a binary classifier is used to verify whether the program matches its claimed name. Specifically, we trained the binary classifier for each known program. Our framework takes a claimed program event data as the input and output the corresponding prediction. The final outputs are +1 or -1 indicating verified or unverified prediction result. 

To train a verification model for a particular program, we collect a set of program events $U=\{e_1, e_2, ..., e_m\}$ including events belong to that program and the ones do not belong to that program. Their corresponding labels are $Y=\{y_1,y_2,...,y_m\}$ with $y_i \in \{+1, -1\}$. If the event data belongs to the claimed program, its ground truth label  $y_i=+1$, otherwise its ground truth label $y_i=-1$.
Our target is to design an end-to-end binary classifier. 
Specifically, we propose to use logistic regression classifier, and the objective function is defined as followed:
\begin{equation}
l=\frac{1}{m}\sum_{i=1}^{m} [y_i\log \hat{y}_i + (1-y_i)\log (1-\hat{y}_i)]
\end{equation}
where $\hat{y}_i$ denotes the predicted label. We optimize the above objective with Adam optimizer. The gradients of the parameters are calculated recursively according to the graph topology. Since our approach is end to end, we directly optimize the reidentification objectives. Once the model achieves a good performance (e.g., using ACC as the measure), the training process terminates, and the trained model is suitable for program reidentification.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Learning Parameters Using Siamese Network}
% In this section, we explain our design of the overall architecture to learn the parameter of proposed model for program re-identification. Specifically, a Siamese Network is proposed in corporate with the previous graph neural networks (GNNs). The Siamese network use two identical GNNs and joint them together. Each GNNs takes a program snapshot as the input and output the corresponding graph embedding $f_{\mathccal{G}}(S)$. The final outputs are the distance of the two graph embeddings $Sim$. Since two GNNs are sharing the same set of parameters, they are identical during the training. The over all architecture is shown in Figure \ref{fig:PL1}

% \begin{figure}[t]
% \centering
% \includegraphics[width = 1\linewidth]{fig/verification.pdf}
% \caption{Parameter Learning Architecture \ours}
% \label{fig:PL1}
% \end{figure}

% Given a set of K pairs of program snapshot $<S_i,S'_{i}>$ with corresponding ground truth pairing information $y_i \in {+1, -1}$, where $y_i=+1$ indicate that $S_i$ and $S'_i$ are belongs to the the program while $y_i=-1$ indicate that $S_i$ and $S'_i$ are belongs to the the different programs. Specifically, we use cosine distance to measure the distance of two embedding. The output of the Siamese network are defined as follow for each pair:
% \begin{equation}
% DIS(S, S')=cos(f_{\mathccal{G}}(S), f_{\mathccal{G}}(S'))=\frac{<f_{\mathccal{G}}(S),f_{\mathccal{G}}(S')>}{||f_{\mathccal{G}}(S)|| \cdot ||f_{\mathccal{G}}(S')||}
% \end{equation}
% To learn the parameters keeps similar embeddings close while pushing dissimilar embeddings apart, we directly optimized the distance between two data points by encourage all positive distance to approach 0, while keeping negative distance about a certain threshold. The objective function is defined as followed:
% \begin{equation}
% l=\sum_{K}^{i=1}(DIS(S,S'_i)-y_i)^2
% \end{equation}
% We optimize the above objective with stochastic gradient descent.
% The gradients of the parameters are calculated recursively according
% to the graph topology. In the end, once the Siamese network
% can achieve a good performance (e.g., using AUC as the measure),
% the training process terminates, and the trained graph embedding
% network can convert an input graph to an effective embedding
% suitable for program re-id.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Parameter Learning via Contrastive Objective}
% In order to train the parameters of the model, we propose a contrastive objective function. To learn graph representation that keeps similar data points close while pushing dissimilar data point apart, we directly optimized the distance between two data points by encourage all positive distance to approach 0, while keeping negative distance about a certain threshold. The constrastive objective is described as followed:
% % \begin{equation}
% % J(\mathcal{H}_G_i,\mathcal{H}_G_j)=y_{ij}D_{ij}^2+(1-y_{ij})[\alpha-D_{ij}]_{+}^2
% % \end{equation}
% \begin{align}
% J(\mathcal{H}_G_i,\mathcal{H}_G_j)=y_{ij}D_{ij}^2+(1-y_{ij})[\alpha-D_{ij}]_{+}^2
% \\
% D_{ij}=||\mathcal{H}_G_i,\mathcal{H}_G_j||
% \label{eq:sp}
% \end{align}
% where $D_{ij}$ denotes the Euclidean distance between two data points. When two data points are in same class, this $y_{ij}=1$. Otherwise $y_{ij}=0$. $\alpha$ indicated the margin.

% \subsection{Parameter Learning via Verification Objective}
% In this section, we explain our design of the overall network architecture to train \ours for Program Re-ID. Specifically, we use the Siamese architecture  

% \subsection{Parameter Learning via Identification Objective}
% In this section, we explain our design of the overall network architecture to train \ours for Program Re-ID 


% \subsection{Parameter Learning via Multi-Task Objective}
% In this section, we explain our design of the overall network architecture to train our \ours Program Re-ID. Specifically, it consists of three stages. First We get the required input program snapshots, then we generate embedding from it via feature learning, finally we optimize it v 

% Behavior of the same program could be much different in different timestamps and machine. Such variation within the same program could overwhelm the variation due to program difference and make program re-id challenging, especially in unconstrained conditions. Thus, it is important to jointly reduce the intra-program variation and enlarge the inter-program difference. It is required that the encoded program representation preserve the propriety that behavior belongs to the same program are close to each other while those of different program should be far away. Therefore, we propose a learning architecture optimized under the supervision of multiple tasks: identification task and verification task to learn such representation. Specifically, identification task formulate the program re-id as a multi-class classification problem, which takes full advantage of the re-ID labels. It directly classifies an input program behavior into a large number of identity classes. 
% %The similarity of two program behavior is computed by the euclidean distance between their embedding
% In the training stage, given an input program behavior with identification supervision, the embedding feature are extracted though feature learning stage and then mapped to one of a large number identities. In the testing stage, the learned embedding feature can be generalized to other task and new identities unseen in the training set. The identification supervision tends to pull separate the different behavior apart and the learned feature embedding would have rich identity-related or inter-program variations. However, the identification supervision has a relatively weak constrain on embedding feature extracted from the same program. Since dissimilar embedding feature could be mapped to the same identity. This could be problematic, when generalize to new task and new identities in the testing stage.
% The verification 


% use both identification and verification signal as supervision.

% handle two type of variation
% the identification task increase the inter-program variation
% the verification task reduce the intra-program variation

% \begin{figure}[t]
% \centering
% \includegraphics[width = 1\linewidth]{fig/Learning_framework_3.pdf}
% \caption{Framework of \ours}
% \label{fig:PL}
% \end{figure}
% In this part, we introduce the conrtastive analysis to learn program similarity/ranking/re-identifcation model. The task of Program Re-ID is to accept or reject the claimed identity of a program. Performance is assessed using two measures: percentage of false accepts
% and the percentage of false rejects. A good system should minimize both measures simultaneously. Following that, we build a trainable system that nonlinearly
% maps the program behavior graph in a low dimensional space so that the distance between these graph is small if the graph belong to the same program and large otherwise. 
% %Specifically, we learning the similarity metric is realized by training
% a network that consists of two identical convolutional
% networks that share the same set of weights -

%the node's current representation $h_v^{k-1}$ is concatenated with the aggregated neighborhood vector. Their concatenated representation is then fed to a fully connected neural network, which generate the representations to be used at the next iteration. In the end, final representation at depth K as $z_v \equiv h^K_v, \forall v \in \mathcal{V}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%

==> bk/04-exp.tex <==
\section{Experiments}
%\myred{Figures??????}

%In this section, we evaluate the proposed method on real system surveillance data collected from a real enterprise network. We first introduce the datasets used on the experiments and the experimental setting. Then we show the effectiveness of the proposed method. We first conduct the synthetic experiment. Then we apply it in  real-world tasks: disguised program detection. Finally, we show the robustness of our approach to the program version upgrade.  
\subsection{Data}
\label{subsec:data}
In the experiments, we evaluate the proposed methods on real-world system monitoring data. The data was collected from a real enterprise network composed of $87$ machines, in a time span of $7$ consecutive weeks. The sheer size of the data set is around 1 Terabytes. We consider three different types of system events as defined in Section~\ref{sec:pre}. Each entity is associated with a set of attributes and each process has a executable name as its identifier/ID. In total, there are about $100$ million event records, with $2000$ processes, $600,000$ files, and $16,412$ Internet sockets. Based on the system event data, we construct the behavior graph (see Section~\ref{subsec:graph}) per program per day. For each entity, we construct three types of features according to Section~\ref{subsec:att}:  \textit{fea-1}: connectivity feature,  \textit{fea-2} statistics feature, and \textit{fea-3}: the combination of \textit{fea-1} and \textit{fea-2}. %For statistic feature, we use four graph measurements, including degree centrality, closeness centrality, betweenness centrality and clustering coefficient .

\nop{
The statistic of the dataset is summarized in Table \ref{tab:dataset}.

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Events       & P-P & P-F & P-I \\ \hline
\#Agent      & 87      & 86       & 84     \\ \hline
\#SEntity    & 1902    & 1935     & 142     \\ \hline
\#DEntity    & 1904    & 69813    & 16466   \\ \hline
\#Edge       & 8    &     &     \\ \hline
\#Avg.Degree &     &     &     \\ \hline
%\#Feature    &     &     &     \\ \hline
\end{tabular}
\caption{The statistics for each type of events}
\label{tab:dataset}
\end{table}
}
\nop{
\myred{check the of Ransomeware}
}
%\vspace{-5pt}
\subsection{Experiment Setup}
\nop{
\subsubsection{Feature Engineering}
For each program entity, we can extract two both connectivity feature and graph statistics feature. In the experiment, we construct three type of features: \textit{fea-1}: connectivity features; \textit{fea-2}: graph statistics features ; \textit{fea-3}: combinations of connectivity features and graph statistics features.
}
\vspace{-5pt}
\subsubsection{Baselines}
To evaluate the performance on \ours, we compare the proposed method with the following typical and state-of-art classification models:
\vspace{-5pt}
\begin{itemize}
\item \textit{LR} and \textit{SVM}: LR and SVM represent the Logistic regression and Linear Support Vector Machine respectively. They are two typical classification methods. The raw features extracted from each process are used as the input, including the connectivity features and the graph statistics feature. The LR amd SVM are implemented use sciket-learn\footnote{http://scikit-learn.org/}.
\vspace{-5pt}
\item \textit{XGB}: XGB represents the gradient boosting. It is a decision tree based classification model implemented using XGBoost\footnote{https://github.com/dmlc/xgboost} \cite{chen2016xgboost}. It is the state-of-art linear classification model in most of tasks. We use maximum $500$ trees with the learning rate equals to 0.1.
\vspace{-5pt}
\item \textit{MLP}: MLP represents the Multi-layer Perceptron, which is a deep neural network based classification model with multiple non-linear layers between the input layer and the output layer. It is a special case of our contextual graph encoder, if we define the propagation layer as identity matrix. 
\end{itemize}

\nop{
Since the proposed approach is based on graph neural network. We compare our method with following graph neural networks methods. 

\begin{itemize}
\nop{
\item \myred{should we compare with traditional node embedding, that's a new work}
}
\item \textit{GCN}:GCN \cite{kipf2016semi} is graph convolutional based semi-supervised classification algorithm. It is a special case of our contextual graph encoder. It consider all the 1-hop neighbourhoods of target entity as the receptive field in each graph encoder and extract the deeper relational feature through stacked multiple convolutional layer. It focus on homogeneous network.
% \item High Uncertainty: There are more than thousand of program in a machine, which causes high uncertainty 
\item \textit{GraphSage}:GraphSage \cite{hamilton2017inductive} is another convolutional-like graph neural network. It is also a special case of our contextual graph encoder. Its receptive field is constructed based on the neighborhood sampled using uniform distribution. It also focus on homogeneous network.

\end{itemize}
}
Since the proposed approach \ourss\ consists of several components, we consider several variations as well. 
\nop{
of our approach, including \textit{\ourss-pp}, \textit{\ourss-pf}, \textit{\ourss-pi}, \textit{\ourss-con}. \textit{\ourss-pp}, \textit{\ourss-pf} and \textit{\ourss-pf} denotes our method only consider single channel. \textit{\ourss-pp} denotes our method consider all channels, but joint different channel with direct concatenation. Our method is implemented with Tensorflow.
}
% \begin{itemize}
% \item \textbf{\ourss-pp}: It is our proposed method only consider P-P channel.
% \item \textbf{\ourss-pf}: It is our proposed method only consider P-F channel.
% \item \textbf{\ourss-pi}: It is our proposed method only consider P-I channel.
% \item \textbf{\ourss-all}: It is our proposed method consider all channels but joint different channel with direct concatenation. 
% \item \textbf{\ourss}: This our proposed method, which consider all channels and joint them together with attentional weight. 
% \end{itemize}
\vspace{-5}
\subsubsection{Evaluation Metrics}
Similar to \cite{Das:2007}\nop{Akoglu:2012}, We evaluate the performance of different methods using a variety of measures, including ACC, F-1 score and AUC score, precision and recall.
% Table 1.

% \begin{table}[]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{|l|l|}
% \hline
% Metrics   & Description                                  \\ \hline
% TP        & \# of target program correctly predicted     \\ \hline
% TN        & \# of other program correctly predicted      \\ \hline
% FP        & \# of false prediction as the target program \\ \hline
% FN        & \# of false prediction as other program      \\ \hline
% %ACC       & (TP+TN)/(TP+TN+FP+FN)                        \\ \hline
% Precision & TP/(TP+FP)                                   \\ \hline
% Recall    & TP/(TP+FN)                                   \\ \hline
% F1        & 2*Precision * Recall/(Precision + Recall)    \\ \hline
% AUC       &                                              \\ \hline
% %TPR       & True positive rate, FP/(TN+FP)               \\ \hline
% %FPR       & False positive rate, FN/(TP+FN)              \\ \hline
% \end{tabular}}
% \caption{Performance metrics}
% \label{tab:metric}
% \end{table}
\vspace{-5}
\subsection{Synthetic Experiments}
In this part, to evaluate the proposed method in a more controlled setting for assessing algorithm performance, we conduct the three sets of synthetic experiments on $500$ most active programs as follows:
(1) we evaluate the effectiveness of multi-layer transformation module and channel-aware attention;%We compare with configuration with single meta-path and their combinations.
\nop{
(2) We evaluate the effectiveness of our proposed contextual neural graph encoder module and compare it with its different variations.
}
(2) we evaluate the performance of our method on normal program reidentification;
(3) we perform the parameter sensitivity analysis.
%We call them synthetic experiments, since all the programs we used in training and testing are normal program with normal behavior. 
%Based on the collected system event data, we first generate one behavior graph per program per time window (\textit{i.e.}, one day). Then, for the target program, we randomly sample $5,00$ behavior graphs generated from different time windows. belonging to that program and another $5,00$ belonging to the rest of programs to have balanced configuration. 
We perform 5-fold cross validation on each program and report the average testing results of all the programs for each evaluation metric. We conduct a grid search on the parameter of each method to identify the parameter setting that yields the highest result, which is done using cross validation. In particular, we set the number of contexts as $100$ and the dimension of hidden layer as $500$.
\vspace{-5pt}
\subsubsection{Evaluation of Different Meta-paths}
In this experiment, %based on the dataset described in Sections 4.1, 
we evaluate the performance of different kinds of meta-paths and their combinations. Given each kind of meta-path, such as P$\rightarrow$P, P$\rightarrow$F or P$\rightarrow$I, corresponding to one type of system event, we construct the multi-channel graph with entity features and then feed them to the contextual graph encoder to generate the graph embedding. After the graph embedding is obtained, we feed it to logistic regression to train the classification model for program reidentification. We denote these baselines as $\ourss_{pp}$, $\ourss_{pf}$, $\ourss_{pi}$, and $\ourss_{con}$. 
%When considering the combination of different meta-paths, we combine the graph embedding generated from different meta-paths. 
For combination of different meta-paths, we consider both direct concatenation and our proposed attentional version, which are denoted as $\ourss_{con}$ and $\ourss_{att}$.
%The experimental results are shown in Table \ref{tab:meta-path}. 
From Table \ref{tab:meta-path}, we can see that different meta-paths and their combinations show different performance, since each of them represents a specific type of dependency. We can also observe that: (1) The $\ourss_{att}$ outperforms all the other meta-paths and their simple combination; (2) The combinations of multiple meta-paths perform better than any single meta-paths, since they cover multiple type of dependency and provide complementary information; (3) The one with channel-aware attention performs better than simple concatenation, since the importance of different meta-paths is different for different programs. Some programs may have active P$\rightarrow$P events, while some one may not. Channel-aware attention captures that difference and computes a weighted combination of different meta-paths; (4) The P$\rightarrow$P and P$\rightarrow$F type meta-paths outperform the $\rightarrow$I type meta-path, since most of programs have active P$\rightarrow$P and P$\rightarrow$F events, while only small part of programs have active P$\rightarrow$I events.

%We use the best selected contextual graph neural encoder in the experiments. 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[htb]
\vspace{-10pt}
\centering
\begin{tabular}{|l|lll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Meta-Path}} & \multicolumn{3}{l|}{Evaluation Criteria} \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                           & ACC          & F-1         & AUC         \\ \hline
$\ourss_{pp}$                                              &    0.838          &    0.864         &     0.843       \\
$\ourss_{pf}$                                              &    0.821          &    0.855         &     0.838       \\
$\ourss_{pi}$                                              &    0.579          &    0.635         &     0.592         \\
$\ourss_{con}$                                          &       0.876       &     0.901        &     0.890        \\
$\ourss_{att}$                                          &       \textbf{0.905}       &     \textbf{0.929}        &     \textbf{0.908}        \\ \hline
\end{tabular}
\caption{Reidentification results of different meta-paths.}
\label{tab:meta-path}
\vspace{-12pt}
\end{table}

\nop{
\subsubsection{Evaluation of Contextual Neural Graph Encoder}
In this set of experiment, we evaluate our proposed contextual neural graph encoder by comparing with several recent graph neural network methods, including the MLP, GCN \cite{kipf2016semi} and GraphSage \cite{hamilton2017inductive}. For MLP, we use use 3 hidden layers (500 neurons in each hidden layer). For GraphSage, we take the best configuration it claimed with pooling aggregation. For all the methods, we stack a two layer neural network. We consider the combination of different meta-path and apply multi-channel translation module and channel-aware attention. The joint graph embedding is generated via different type of graph neural networks. The logistic regression is used as the classification model for all the methods.  
The verification results of different graph representation learning methods are shown in Table \ref{tab:ge}
From Table \ref{tab:ge} we can see that the proposed CGE outperfoms all the other all baseline for program verification in terms of all the metrics. That is to say, CGE learns effective program representation than current state-of-art methods. The success CGE les in the proper consideration and accommodation of the directed link in the graph. Further more, we can see that the MLP has worst performance, since it only use the entity attributes and ignore the structure information. The performance of GCN slightly outperform GraphSage, due to its wider receptive field. 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{|l|lll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{l|}{Evaluation Criteria} \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & ACC & F-1 & AUC \\ \hline
MLP &0.778  &0.808  &0.780  \\
GCN &0.891  &0.910  &0.899  \\
GraphSage &0.888  &0.898  &0.891  \\
CGE &\textbf{0.905}  & \textbf{0.929}  & \textbf{0.908} \\ \hline
\end{tabular}
\caption{Comparisons of CGE with other network representation learning methods in program verification.}
\label{tab:ge}
\end{table}
}
\vspace{-5pt}
\subsubsection{Evaluation on Normal Program Reidentification}
In this set of experiments, we evaluate the performance on normal program reidenfitication by comparing our method with other four baselines including LR, SVM, XGB and MLP. We use the constructed features as described in Section~\ref{subsec:data}. %Based on these features, we consider four typical classification models, i.e., Logistical Regression, SVM, XGB and MLP. Among them XGB is the most powerful and scalable classification model. MLP is a typical neural network based model. 
To show the effectiveness of the deep learning model, we consider both shallow and deep version of neural network based model, which is denoted as $"XXX_{shallow}"$ and $"XXX_{deep}"$, respectively. We consider only one layer of neural network in the shallow model, and three layers for the deep model. For the baseline methods, we use the constructed raw features: \textit{fea-1}, \textit{fea-2}, \textit{fea-3} as the input.
The experimental results are illustrated in Table \ref{tab:overall}. From the results, we can observe that the proposed \ourss\ consistently and significantly outperform all baselines in terms of all metrics. The Table \ref{tab:overall} also shows that: (1) \textit{fea-3}(concatenate the connectivity feature and graph statistic feature) helps the performance for all baseline classification model, but since they are all raw feature without considering graph structure, their performance can not capture up with the proposed method; (2) \textit{fea-2}(graph statistic feature) is more useful than \textit{fea-1}(graph connectivity feature), since \textit{fea-1} is very sparse, which is difficult to use for some state-of-art methods, such as SVM; (3) the deep model outperforms the shallow model for deep learning method, since deep model can capture the hierarchical representation of the raw feature. 


\begin{table*}[]
\small
\centering
\vspace{-15pt}
\begin{tabular}{|l|l|lllll}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{Settings} & \multicolumn{5}{l|}{Evaluation Criteria} \\ \cline{3-7} 
\multicolumn{1}{|c|}{} &  & ACC & F-1 & AUC & Precision & \multicolumn{1}{l|}{Recall} \\ \hline
\multirow{3}{*}{LR} & \textit{fea-1} &0.693  & 0.755 & 0.699  &0.632  & \multicolumn{1}{l|}{0.948} \\
 & \textit{fea-2} & 0.705 & 0.770 & 0.703  & 0.655 & \multicolumn{1}{l|}{0.950} \\
 & \textit{fea-3} & 0.724 & 0.772 & 0.727 & 0.675 & \multicolumn{1}{l|}{0.948} \\ \hline
\multirow{3}{*}{SVM} & \textit{fea-1} &0.502  &0.662  &0.502  &0.505 & \multicolumn{1}{l|}{0.970} \\
 & \textit{fea-2} & 0.795 & 0.778 & 0.725 & 0.701 & \multicolumn{1}{l|}{0.935} \\
 & \textit{fea-3} & 0.504 & 0.652 & 0.504 & 0.505 & \multicolumn{1}{l|}{\textbf{0.975}} \\ \hline
\multirow{3}{*}{XGB} & \textit{fea-1} & 0.775  & 0.802 & 0.776 & 0.732 &  \multicolumn{1}{l|}{0.930} \\
 & \textit{fea-2} & 0.833 & 0.860 & 0.846 & 0.821 & \multicolumn{1}{l|}{0.936} \\
 & \textit{fea-3} & 0.855 & 0.866 & 0.856 & 0.827 & \multicolumn{1}{l|}{0.937} \\ \hline
\multirow{3}{*}{MLP_{shallow}} & \textit{fea-1} &0.633  & 0.745 & 0.643 & 0.626 & \multicolumn{1}{l|}{0.938} \\
 & \textit{fea-2} & 0.775 & 0.808 & 0.779 & 0.724  & \multicolumn{1}{l|}{0.932} \\
 & \textit{fea-3} & 0.778 & 0.808 & 0.780 & 0.726 &  \multicolumn{1}{l|}{0.932} \\ \hline
\multirow{3}{*}{MLP_{deep}} & \textit{fea-1} & 0.633  & 0.743  & 0.653  & 0.625  & \multicolumn{1}{l|}{0.945} \\
 & \textit{fea-2} & 0.801 & 0.830  & 0.805   & 0.769 & \multicolumn{1}{l|}{0.921} \\
 & \textit{fea-3} & 0.815 & 0.831 & 0.816 & 0.778 & \multicolumn{1}{l|}{0.923} \\ \hline
\ourss_{shallow} & / & 0.905 & 0.929 & 0.908 & 0.905 & \multicolumn{1}{l|}{0.933} \\
\ourss_{deep} & / & \textbf{0.929} & \textbf{0.961} & \textbf{0.935} & \textbf{0.932} & \multicolumn{1}{l|}{0.936} \\ \hline
\end{tabular}
\caption{Comparison of other classification methods.}
\label{tab:overall}
\vspace{-10pt}
\end{table*}

\vspace{-5pt}
\subsubsection{Parameter Sensitivity}
In this experiment, we conduct the sensitivity analysis of how different choices of parameters will affect the performance of our proposed approach. Specifically, our approach has two important parameters: the number of context in each propagation layer and the number of dimension in each proceptron layer. The results are shown in Figure \ref{fig:p_cont} and \ref{fig:p_dim}.

\begin{figure}[htb]
\vspace{-10pt}
\centering
 \subfigure[\# contexts vs. ACC]{\label{fig:p_cont}
    \begin{minipage}[l]{0.45\linewidth}
     \centering
     \includegraphics[width=\linewidth]{fig/P_CON.pdf}
    \end{minipage}
 }~
 \subfigure[\# dimensions vs. ACC]{\label{fig:p_dim}
    \begin{minipage}[l]{0.45\linewidth}
     \centering
     \includegraphics[width=\linewidth]{fig/P_DIM.pdf}
    \end{minipage}
 }
\caption{Parameter sensitivity evaluation.}\label{fig:exp_comp1}
\vspace{-15pt}
\end{figure}


\vspace{-5pt}
\subsection{Real-word Experiment}
In this section, we evaluate the performance of the \ourss\ in two real-world tasks: disguised program detection and program version upgrade detection.
\vspace{-5pt}
\subsubsection{Disguised Program Detection}
In the real-world computer system, the hacker usually disguise their malicious program as the normal program to bypass the anit-virus software. It is important to verify whether the program is real or not.

In this experiment, %we use \ourss\ in a real-world disguised program detection task. 
we simulate five different types of real attacks as described below: 
(1) \textit{WannaCry}: A cryptoworm which disguised itself as 7z.exe.
(2) \textit{Phishing Email}: A malicious Trojan was downloaded as an Outlook attachment and the enclosed macro was triggered by Excel to create a fake java.exe, and the disguised malicious java.exe further SQL exploited a vulnerable server to start cmd.exe in order to create an info-stealer.
(3) \textit{Emulating Enterprise Environment}: The hacker generate telnet process to create malware binary(trojan.exe). Then, trojan exe is created to connect back to hackers and DLL is injected through the running process notepad.exe. The hackers use mimikaz and kiwi for memory operation inside the meterpreter context. Finally, malware PwDump7.exe and wce.exe are copied and run on target hosts.
(4) \textit{Diversifying Attack Vectors}: The attacker first writes malicious PHP file by HTTP connection, then downloads the malware process(trojan.exe), and connects back to attack host. The process notepad.exe is run to perform DLL injection. Hacker further use mimikaza and kiwi to perform memory operation inside meterpreter context. Finally, it copies and runs Pwdup7.exe and wce.exe on the target host.
(5) \textit{Domain Controller Penetration} The hacker first sends an email attaching a document that includes the malware python32.exe. This malware opens a connection back to the attacker so that they can run notepad.exe and perform reflective DLL injection to obtain need privileges. Then, they transfer password enumerator and run the process gsecdumpv2b5.exe to get all user credentials. Finally, they probe the SQL server address and dump the database into their own bases. We tried each type of the attack ten times during different time windows to generate different testing samples.

%In our experiment, it detects the disguised program by identifying if its behavior matches its claimed name. 
The detection performance is evaluated by the true positive rate (TPR) and false positive rate (FPR). 
The TPR defines the fraction of intrusion attacks that are detected during the evaluation. FPR, on the other hand, describes the fraction of normal event sequences that trigger an alert during the evaluation. We compare our method with the four baselines, and use the deep model for all neural network based methods. Figure \ref{fig:real1} shows that \ourss\ outperform all the other baselines by at least $12\%$ in TPR and $10\%$ in FPR.% in recall
%The TP means the number of truly disguised program detected by the \ourss\ while the FP means the number of truly disguised program undetected. 
%The short description of each ATP attacks, with corresponding detection result is shown in Table \ref{tab:real1}.
\begin{figure}[htb]
\vspace{-10pt}
\centering
 \subfigure[TPR]{\label{fig:real1_TPR}
    \begin{minipage}[l]{0.45\linewidth}
     \centering
     \includegraphics[width=\linewidth]{fig/TPR.pdf}
    \end{minipage}
 }~
 \subfigure[FPR]{\label{fig:real2_FPR}
    \begin{minipage}[l]{0.45\linewidth}
     \centering
     \includegraphics[width=\linewidth]{fig/FPR.pdf}
    \end{minipage}
 }
\caption{Disguised Program Detection Results.}\label{fig:real1}
\vspace{-15pt}
\end{figure}

% \begin{figure}[htb]
% \centering
% \vspace{-5pt}
% \includegraphics[width = 0.8\linewidth]{fig/real_1.pdf}
% \vspace{-5pt}
% \caption{Disguised Program Detection Results.}
% \label{fig:real-1}
% \vspace{-15pt}
% \end{figure}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\nop{
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{Attacks} & \multirow{2}{*}{Short Description}                                                                                                                                                                                                                                                                          & \multicolumn{2}{l|}{Evaluations} \\ \cline{3-4} 
                         &                                                                                                                                                                                                                                                                                                             & TP               & FP            \\ \hline
WannaCry                 & A cryptoworm which disguised its tasksche.exe as 7z.exe.                                                                                                                                                                                                                   & 98\%            & 0\%           \\ \hline
% Phishing Email           & \begin{tabular}[c]{@{}l@{}}A malicious Trojan was downloaded as an Outlook attachment and the  \\enclosed macro was triggered by Excel to create a fake java.exe, and the   \\ malicious java.exe further SQL exploited a vulnerable server to start  \\cmd.exe in order to create an info-stealer\end{tabular} & 100\%            & 0\%           \\ \hline
Phishing Email           & \begin{tabular}[c]{@{}l@{}}Hacker create a fake java.exe. \end{tabular} & 100\%            & 0\%           \\ \hline
\begin{tabular}[c]{@{}l@{}}Emulating \\Enterprise\\ Environment\end{tabular} & \begin{tabular}[c]{@{}l@{}}The hacker disguised trojan.exe as notepad.exe \end{tabular}                                                                                             & 100\%            & 0\%           \\ \hline
%\begin{tabular}[c]{@{}l@{}}Emulating \\Enterprise\\ Environment\end{tabular} & \begin{tabular}[c]{@{}l@{}}The hacker generate telnet process to create malware binary(trojan.exe). \\then, trojan exe is created to connect back to hackers and DLL is injected  \\through the running process notepad.exe. The hackers use mimikaz and \\ kiwi for memory operation inside the meterpreter context.  Finally, \\malware PwDump7.exe and wce.exe are copied and run on target hosts.\end{tabular}                                                                                             & 100\%            & 0\%           \\ \hline
% \begin{tabular}[c]{@{}l@{}}Diversifying \\Attack\\ Vectors \end{tabular} & \begin{tabular}[c]{@{}l@{}}The attacker first writes malicious PHP file by HTTP connection, then \\downloads the malware process(trojan.exe), and connects back to attack \\host. The process notepad.exe is run to perfrom DLL injection. Hacker \\ further use mimikaza and kiwi to perform memory operation inside \\meterpreter context. Finally, it copys and runs Pwdup7.exe and wce.exe \\on the target host. \end{tabular}                                                                                             & 100\%            & 0\%           \\ \hline
\begin{tabular}[c]{@{}l@{}}Diversifying \\Attack\\ Vectors \end{tabular} & \begin{tabular}[c]{@{}l@{}}The attacker disguised trojan.exe as notepad.exe\end{tabular}                                                                                             & 100\%            & 0\%           \\ \hline
\begin{tabular}[c]{@{}l@{}}Domain\\ Controller\\Penetration    \end{tabular}      & \begin{tabular}[c]{@{}l@{}}The hacker disguised malware as python32.exe\end{tabular}                                                                                             & 100\%            & 0\%           \\ \hline
% Netcat Backdoor          & \begin{tabular}[c]{@{}l@{}}An attack downloaded the netcat utility and used it to open a Backdoor, \\from which a Persistent Netcat port scanner was then downloaded and  \\executed using PowerShell\end{tabular}                                                                                             & 100\%            & 0\%           \\ \hline
% Cheating Student         & \begin{tabular}[c]{@{}l@{}}A student downloaded midterm scores from Apache, and uploaded a  \\modified version \end{tabular}                                                                                                                                                                                                                           & 100\%            & 0\%           \\ \hline
% Passing the Hash         & \begin{tabular}[c]{@{}l@{}}An attack connected to Windows domain Controller using PsExec and run \\credential dumper \end{tabular}                                                                                                                                                                                                                    & 100\%            & 0\%           \\ \hline
\end{tabular}
\caption{Real-world attack scenarios with short description and detection results 
\nop{\myred{Current short description does not make sense. I do not think Cheating Student is a good case for our story. Using some cases from the slides I sent to you. And focus on describing which program has been disguised as which normal program. For the numbers, how can the TP always be 100\% and FP always be 0\%? Try to get the real numbers. For the cases we do not have the data, try to download the malware and ask security team to help you run in the malware lab.}}}
\label{tab:real1}
\end{table}
}

\subsubsection{Robustness Study on Program Upgrade}
The normal program usually get upgrade with multiple versions. However, different versions have different signatures, which may cause false alarms in intrusion detection systems.
In this experiment, we evaluate the robustness of \ourss\ on program upgrade. In particular, we select the CHROME.EXE for case study. We collect the data of CHROME.EXE with three different versions and and one version of WINWORD.EXE. Then, the embedding before the classifier for these CHROME.EXE data and WINWORD.EXE data are extracted and visualized using t-SNE. The result is shown in Figure \ref{fig:t-sne}. We can see that in the embedding space, the data points belongs to the different versions of CHROME.EXE are close to each other, even they have different signatures, while the data points of WINWORD.EXE are far away from the CHROME.EXE, which demonstrate our method is robust to the normal program upgrade.   
\begin{figure}[htb]
\vspace{-10pt}
\centering
\includegraphics[width = 1\linewidth]{fig/T-SNE.pdf}
\caption{Scatter plot embedding of different versions of CHROME.EXE vs WINWORD.EXE.}
\label{fig:t-sne}
\vspace{-15pt}
\end{figure}
%\myred{TODO: add embedding visualization}

% \begin{table}[]
% \centering
% \begin{tabular}{|c|c|cccc|}
% \hline
% \multirow{2}{*}{Channel} & \multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{Evalution Criteria}                                                                         \\ \cline{3-6} 
%                          &                            & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F-1} & AUC                   \\ \hline
% \multirow{7}{*}{P-P}     & LR                         & 80                             & 80                          & 80                       & 80                    \\
%                          & SVM                        &                                &                             &                          &                       \\
%                          & XGB                        &                                &                             &                          &                       \\
%                          & MLP                        &                                &                             &                          &                       \\
%                          & GCN                        &                                &                             &                          &                       \\
%                          & Ours\_pp\_c                & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}     & \multicolumn{1}{l|}{} \\
%                          & Ours\_pp                   &                                &                             &                          &                       \\ \hline
% \multirow{7}{*}{P-F}     & LR                         &                                &                             &                          &                       \\
%                          & SVM                        &                                &                             &                          &                       \\
%                          & XGB                        &                                &                             &                          &                       \\
%                          & MLP                        &                                &                             &                          &                       \\
%                          & GCN                        &                                &                             &                          &                       \\
%                          & Ours\_pf\_c                & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}     & \multicolumn{1}{l|}{} \\
%                          & Ours\_pf                   &                                &                             &                          &                       \\ \hline
% \multirow{7}{*}{P-I}     & LR                         &                                &                             &                          &                       \\
%                          & SVM                        &                                &                             &                          &                       \\
%                          & XGB                        &                                &                             &                          &                       \\
%                          & MLP                        &                                &                             &                          &                       \\
%                          & GCN                        &                                &                             &                          &                       \\
%                          & Ours\_pi\_c                &                                &                             &                          &                       \\
%                          & Ours\_pi                   &                                &                             &                          &                       \\ \hline
% \multirow{9}{*}{All}     & LR                         &                                &                             &                          &                       \\
%                          & SVM                        &                                &                             &                          &                       \\
%                          & XGB                        &                                &                             &                          &                       \\
%                          & MLP                        &                                &                             &                          &                       \\
%                          & GCN                        &                                &                             &                          &                       \\ \cline{2-6} 
%                          & Ours\_noAttn\_c            &                                &                             &                          &                       \\
%                          & Ours\_noAttn               &                                &                             &                          &                       \\
%                          & Ours\_c                    &                                &                             &                          &                       \\
%                          & Ours                       &                                &                             &                          &                       \\ \hline
% \end{tabular}
% \caption{My caption}
% \label{my-label}
% \end{table}

% \begin{table}[]
% \small
% \centering
% \begin{tabular}{|c|c|cccc|}
% \hline
% \multirow{2}{*}{Channel}      & \multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{Evalution Criteria}                                                       \\ \cline{3-6} 
%                               &                            & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F-1} & AUC \\ \hline
% \multirow{6}{*}{P-P}           & LR                         & 80                             & 80                          & 80                       & 80  \\
%                               & SVM                        &                                &                             &                          &     \\
%                               & XGB                        &                                &                             &                          &     \\
%                               & MLP                        &                                &                             &                          &     \\
%                               & GCN                        &                                &                             &                          &     \\
%                               & Ours\_pp                   &                                &                             &                          &     \\ \hline
% \multirow{6}{*}{P-F}           & LR                         &                                &                             &                          &     \\
%                               & SVM                        &                                &                             &                          &     \\
%                               & XGB                        &                                &                             &                          &     \\
%                               & MLP                        &                                &                             &                          &     \\
%                               & GCN                        &                                &                             &                          &     \\
%                               & Ours\_pf                   &                                &                             &                          &     \\ \hline
% \multirow{6}{*}{P-I}           & LR                         &                                &                             &                          &     \\
%                               & SVM                        &                                &                             &                          &     \\
%                               & XGB                        &                                &                             &                          &     \\
%                               & MLP                        &                                &                             &                          &     \\
%                               & GCN                        &                                &                             &                          &     \\
%                               & Ours\_pi                   &                                &                             &                          &     \\ \hline
% \multirow{7}{*}{ALL}           & LR                         &                                &                             &                          &     \\
%                               & SVM                        &                                &                             &                          &     \\
%                               & XGB                        &                                &                             &                          &     \\
%                               & MLP                        &                                &                             &                          &     \\
%                               & GCN                        &                                &                             &                          &     \\ \cline{2-6} 
%                               & Ours\_noAttn               &                                &                             &                          &     \\
%                               & Ours                       &                                &                             &                          &     \\ \hline
% \end{tabular}
% \caption{My caption}
% \label{tab:}
% \end{table}

% \begin{table}[]
% \centering
% \small
% \begin{tabular}{|c|c|cccc|}
% \hline
% \multirow{2}{*}{Channel} & \multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{Evalution Criteria}                                                       \\ \cline{3-6} 
%                          &                            & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F-1} & AUC \\ \hline
% \multirow{8}{*}{P-P}     & LR                         & 80                             & 80                          & 80                       & 80  \\
%                          & SVM                        &                                &                             &                          &     \\
%                          & XGB                        &                                &                             &                          &     \\
%                          & MLP                        &                                &                             &                          &     \\
%                          & GCN                        &                                &                             &                          &     \\
%                          & Ours\_pp\_r1               &                                &                             &                          &     \\
%                          & Ours\_pp\_r2               &                                &                             &                          &     \\
%                          & Ours\_pp\_r3               &                                &                             &                          &     \\ \hline
% \multirow{8}{*}{P-F}     & LR                         &                                &                             &                          &     \\
%                          & SVM                        &                                &                             &                          &     \\
%                          & XGB                        &                                &                             &                          &     \\
%                          & MLP                        &                                &                             &                          &     \\
%                          & GCN                        &                                &                             &                          &     \\
%                          & Ours\_pp\_r1               &                                &                             &                          &     \\
%                          & Ours\_pp\_r2               &                                &                             &                          &     \\
%                          & Ours\_pp\_r2               &                                &                             &                          &     \\ \hline
% \multirow{8}{*}{P-I}     & LR                         &                                &                             &                          &     \\
%                          & SVM                        &                                &                             &                          &     \\
%                          & XGB                        &                                &                             &                          &     \\
%                          & MLP                        &                                &                             &                          &     \\
%                          & GCN                        &                                &                             &                          &     \\
%                          & Ours\_pi\_1                &                                &                             &                          &     \\
%                          & Ours\_pi\_2                &                                &                             &                          &     \\
%                          & Ours\_pi\_3                &                                &                             &                          &     \\ \hline
% \multirow{11}{*}{All}    & LR                         &                                &                             &                          &     \\
%                          & SVM                        &                                &                             &                          &     \\
%                          & XGB                        &                                &                             &                          &     \\
%                          & MLP                        &                                &                             &                          &     \\
%                          & GCN                        &                                &                             &                          &     \\ \cline{2-6} 
%                          & Ours\_noAttn\_r1           &                                &                             &                          &     \\
%                          & Ours\_noAttn\_r2           &                                &                             &                          &     \\
%                          & Ours\_noAttn\_r3           &                                &                             &                          &     \\
%                          & Ours\_r1                   &                                &                             &                          &     \\
%                          & Ours\_r2                   &                                &                             &                          &     \\
%                          & Ours\_r3                   &                                &                             &                          &     \\ \hline
% \end{tabular}
% \caption{My caption}
% \label{my-label}
% \end{table}


% \subsection{Malware Detection}

% \begin{table}[]
% \centering
% \begin{tabular}{|c|cccc|}
% \hline
% \multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{Evalution Criteria}                                                       \\ \cline{2-5} 
%                           & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F-1} & AUC \\ \hline
% LR                         &                                &                             &                          &     \\
% SVM                        &                                &                             &                          &     \\
% XGB                        &                                &                             &                          &     \\
% MLP                        &                                &                             &                          &     \\
% GCN                        &                                &                             &                          &     \\ \hline
% Ours\_noAttn               &                                &                             &                          &     \\
% Ours                       &                                &                             &                          &     \\ \hline
% \end{tabular}
% \caption{My caption}
% \label{my-label}
% \end{table}

% \subsection{Case Study for Signature Diversity}

% \begin{table}[]
% \centering
% \begin{tabular}{|c|cccc|}
% \hline
% \multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{Evalution Criteria}                                                       \\ \cline{2-5} 
%                           & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F-1} & AUC \\ \hline
% LR                         &                                &                             &                          &     \\
% SVM                        &                                &                             &                          &     \\
% XGB                        &                                &                             &                          &     \\
% MLP                        &                                &                             &                          &     \\
% GCN                        &                                &                             &                          &     \\ \hline
% Ours\_noAttn               &                                &                             &                          &     \\
% Ours                       &                                &                             &                          &     \\ \hline
% \end{tabular}
% \caption{My caption}
% \label{my-label}
% \end{table}

% \subsection{Attention Weight}

==> bk/05-related.tex <==
\section{Related Work}
%Our work is related to Intrusion Detection and Graph Representation Learning. We briefly discuss them in the followings.

\subsection{Intrusion Detection}
\nop{
The malicious program detection powered by machine Learning and data mining is an emerging research topic due to the increasing number of malicious programs and the developing the of the AI algorithm. There are a number work are proposed based on the machine learning and data mining \cite{arp2014drebin,dimjavsevic2016evaluation,wu2014droiddolphin,saleh2017multi,hou2017hindroid}. These work follow a two-stage pipeline and formulate the malicious program detection as a binary classification problem. They first extract the feature from the malware samples and then perform binary classification using different classifier, such as K-NN, Naive Bayesian, Decision Tree and SVM. More recently, a number of works adopt the deep learning to perform this pipeline end-to-end. \cite{saxe2015deep} proposes to use Auto-Encoder and Deep Belief Network to extract hidden representation as the signature of the malware. 
\cite{david2015deepsign} combines the deep neural network and Bayesian Calibrate Model.
\cite{hardy2016dl4md} proposes SAEs based deep learning architecture to learn from Windows API calls for malware detection.
Different from previous work, our work is in a general view, which has broader applications, including Malicious Program Detection. 
}

In general, intrusion detection refers to the process of monitoring the events occurring in a computer system or network, and analyzing them for signs of intrusions. Currently there are two basic approaches to intrusion detection, namely anomaly detection and misuse detection \cite{jones2000computer}. Anomaly detection approaches define and characterize correct/wrong behaviors of the system, while the misuse detection approaches monitor for explicit patterns, with the intrusion patterns known in advance.
%\noindent \textbf{Anomaly Detection.} 
Existing anomaly detection approaches in large-scale enterprise network systems have been separately considering different data representations. In particular, host-based anomaly detection methods locally extracted patterns from process-level events as the discriminators of abnormal intrusion \cite{hofmeyr1998intrusion,mutz2006anomalous}. In contrast, network-based anomaly detection methods focused on disclosing abnormal subgraph structures from network-level events, most of which were inspired by graph properties \cite{noble2003graph}.%\cite{ide2004eigenspace,noble2003graph}. %All these related work, however, did not take into account both types of events together. Different from these work, we consider the heterogeneity among data.
\vspace{-5pt}
\subsection{Representation Learning for Graph Classification}
Recently Representation Learning \cite{bengio2013representation} has long been an important problem of machine learning and many works aim at learning representations with deep learning due to its powerful ability of learning feature with different kinds properties. Recent years, several deep learning approaches are proposed on graph-structured data, including \cite{kipf2016semi,defferrard2016convolutional,bruna2013spectral,hamilton2017inductive,velickovic2017graph}. They leverage convolution operation in spatial domain to approximate the convolution operation in spectral domain. \cite{defferrard2016convolutional,bruna2013spectral} propose the fast localized convolutions. \cite{kipf2016semi} propose a first order approximation scheme to reduce the computation cost of graph filter spectrum. \cite{hamilton2017inductive} extends the the graph convolution with a more general form of sample and aggregation function for node context. A more recent work by \cite{velickovic2017graph} learns the context aggregation with considering the weights between the neighbourhood and current nodes. 
However these work mainly focus on the node classification. Different from theirs, our work focus on the graph embedding. Further more, we embed the graph in an attentional multi-channel neural network framework. 
%Malware detection
% In order to keep combating the increasing number of malicious programs, there have been a number of research works on developing malicious program detection system using machine learning and data mining methods \cite{david2015deepsign,saleh2017multi,arp2014drebin,hou2017hindroid,dimjavsevic2016evaluation,wu2014droiddolphin}. The main difference among these works are how features are extracted from the program. They can be categorized into two types. 
% One type is to perform static analysis and extract 
% One type is to perform dynamic analysis and extract dynamic features through debugger, simulator, emulator and VM. For example, \cite{wu2014droiddolphin} use Droidbox and APE to record thirteen activities. Another example is 

% On type is to use 

% However, in the real-world problem 

% % Android Malware Detection using Large-scale Network Representation Learning 

% the system have to see the malware of same family
% The log is a very low quality input, Unstructured information  structure: very hard

% focus on feature retrieval: most are already used in security paper

% Simplified problem: not an unseen malware, but the variant from the same family
% The one with same/very similar features are already in training set  
% The result will be always be good on whatever features or algorithms
% Overfitting, or more seriously, cheating

% 21.   Rule 21: Related work: Categorize the related work, instead of pointing directly the problems/flaws of a specific work with name, discuss the general problems of the category and why these works cannot be applied to the proposed problem. If possible, provide a summary table in the end, to compare the features of related work with the proposed methods.

==> bk/06-conclusion.tex <==
\section{Conclusion}
\nop{
In this paper, we propose the problem of program verification via deep graph neural network in a data driven manner.
\myred{Rewrite the conclusion. Conclusion should be totally different to the abstract.}
In this paper, we propose a graph neural network based method (\ourss) to verify the program based on its monitoring and surveillance data. The key idea is to leverage the representation learning of the program behavior graph to guide the verification process. We formulate this problem from a graph classification perspective, and develop an effective multi-channel attentional graph embedding algorithm to solve it. Extensive experiments --- using real-world enterprise monitoring data and real attacks --- show that \ourss\ is effective in identifying the disguised signed programs and robust to the normal dynamic changes like program version upgrade.
}

In this paper, we investigate the problem of program re-identification in IT/OT systems, which is often overlooked by traditional intrusion detection techniques. We propose \ourss, an attentional graph neural network method to verify the program's identity based on its behavior graph. %\ourss\ is the first deep learning framework for graph classification task on heterogeneous directed graphs. 
%We address the challenge to leverage the system monitoring data. 
Different from the existing graph neural network methods, \ourss\ is able to capture and encode the heterogeneous complex dependency among different entities in a hierarchical way. The experimental results show that \ourss\ outperforms all the baseline methods by at least $10\%$ in terms of all the metrics. 
We also apply \ourss\ to a real enterprise system for disguised program detection. Our method can achieve superior performance and demonstrate robustness to the normal dynamic changes. 

%The real-world experiments show that \ourss\ the effectiveness in identifying the disguised signed programs and robust to the normal dynamic changes like program version upgrade.    



% to . A multi-channel transformation module is developed to translate the heterogeneous graph to multiple channels of homogeneous graph. A contextual graph encoder is then proposed to extract the graph embedding preserving the directed dependency. A channel-aware attention module is designed to align the graph embedding from different channels. 
% We implement and deploy our approach to a real enterprise security system, and evaluate the proposed algorithm
% in extensive experiments. The experiment results convince us of the effectiveness and efficiency of our approach.
